Mildly Exponential Lower Bounds on Tolerant Testers for Monotonicity, Unateness, and Juntas

We give the first super-polynomial (in fact, mildly exponential) lower bounds for tolerant testing (equivalently, distance estimation) of monotonicity, unateness, and juntas with a constant separation between the "yes" and "no" cases. Specifically, we give $\bullet$ A $2^{\Omega(n^{1/4}/\sqrt{\varepsilon})}$-query lower bound for non-adaptive, two-sided tolerant monotonicity testers and unateness testers when the "gap" parameter $\varepsilon_2-\varepsilon_1$ is equal to $\varepsilon$, for any $\varepsilon \geq 1/\sqrt{n}$; $\bullet$ A $2^{\Omega(k^{1/2})}$-query lower bound for non-adaptive, two-sided tolerant junta testers when the gap parameter is an absolute constant. In the constant-gap regime no non-trivial prior lower bound was known for monotonicity, the best prior lower bound known for unateness was $\tilde{\Omega}(n^{3/2})$ queries, and the best prior lower bound known for juntas was $\mathrm{poly}(k)$ queries.

==> images/junta.tex <==
%!TEX root = ../tolerant.tex

%\begin{figure}
%
%\begin{tikzpicture}
%	
%\end{tikzpicture}
%
%\caption{Do we want a junta figure as well? \red{{\bf Rocco:} Maybe we're okay without a junta figure?}}
%\label{fig:junta}
%	
%\end{figure}


==> images/monotone-n.tex <==
%!TEX root = ../tolerant.tex
%
%\usetikzlibrary{decorations.pathreplacing,angles,quotes}
%\usetikzlibrary{shapes.geometric}
%\usetikzlibrary{patterns}
%
%\begin{figure}
%
%\centering
%
%\begin{tikzpicture}[scale=0.86]
%
%	%%%%%%%%%%%%%%% CONTROL SUBCUBE %%%%%%%%%%%%%%%%% 
%	
%	% colors
%	\fill[pattern= crosshatch,pattern color=black, opacity=0.25] (-1, -1.5) -- (-0.5, -1) -- (-2.25, 0.75) -- (-2.75, 0.25);
%	\fill[pattern= crosshatch,pattern color=black, opacity=0.25] (1, -1.5) -- (0.5, -1) -- (2.25, 0.75) -- (2.75, 0.25);
%%	\fill[pattern=north west lines,pattern color=black, opacity=0.5] (-0.5, -1) -- (0, -1.5) -- (0.5, -1) -- (0, -0.5);
%	
%	\fill[color=purple!20!blue!40!white!70] (-2.25, 0.75) -- (-0.5, -1) -- (0, -0.5) -- (0.5, -1) -- (2.25, 0.75) -- (0, 3);
%	\fill[color=purple!20!blue!40!white!70] (-2.5, 0.5) -- (0, 3) -- (2.5, 0.5);
%	
%	\fill[color=white] (-3, 0) -- (0, -3) -- (3, 0); 
%	
%	% control cube
%	\draw[-] (0, -3) -- (-3, 0) -- (0, 3) -- (3, 0) -- (0, -3);
%	\draw[dashed] (-3, 0) -- (3, 0);
%	\draw[dashed] (-2.5, 0.5) -- (2.5, 0.5);
%
%	
%	% talagrand subcubes
%	\draw[-] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25);
%	\draw[-] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75);
%	\draw[-,line width=0.3mm] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
%		
%	% nodes
%	\node (0) at (0, -2){$0$};
%	\node (1) at (0, 1){$1$};
%	\node (talagrand-cube) at (1.15, -0.85){$\bT_{\ell}$};
%	
%%	\node (blah) at (-3.75, 0){$|x| = \frac{m}{2}$};
%%	\node (bleh) at (-4.25, 0.5){$|x| = \frac{m + 0.1\eps\sqrt{m}}{2}$};
%	
%	\draw[decoration={brace,raise=5pt,}, decorate, line width=0.25mm] (-3.05, 0) -- node[left=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{m}{2}, \frac{m + 0.1\eps\sqrt{m}}{2}}$} (-3.05, 0.5);
%	
%	
%	%%%%%%%%%%%%%%%% ACTION SUBCUBES %%%%%%%%%%%%%%%%%
%	
%	% top
%	
%	\node (heads) at (5.5, 2.5){\includegraphics[width=1.1cm]{images/quarter-front}};
%	\node (bh) at (5.5, 1.5){If $\bb_{\ell} = 1$:};
%	
%	\fill[color=purple!20!blue!40!white!70] (10, 2) -- (9, 1) -- (8, 2);
%	
%	\draw[-] (9, 1) -- (7.5, 2.5) -- (9, 4) -- (10.5, 2.5) -- (9, 1);
%	\draw[dashed] (10, 2) -- (8, 2);
%	\draw[dashed] (10, 3) -- (8, 3);
%	
%	\node() at (9, 3.4){$0$};
%	\node() at (9, 2.5){$0$};
%	\node() at (9, 1.6){$1$};
%	
%	% bottom
%	
%	\node (tails) at (5.5, -2){\includegraphics[width=1.1cm]{images/quarter-back}};
%	\node (bt) at (5.5, -3){If $\bb_{\ell} = 0$:};
%	
%	\fill[color=purple!20!blue!40!white!70] (10, -1.5) -- (9, -0.5) -- (8, -1.5);
%	
%	\draw[-] (9, -3.5) -- (7.5, -2) -- (9, -0.5) -- (10.5, -2) -- (9, -3.5);	
%	\draw[dashed] (10, -2.5) -- (8, -2.5);
%	\draw[dashed] (10, -1.5) -- (8, -1.5);
%	
%	\node() at (9, -1.1){$1$};
%	\node() at (9, -2){$0$};
%	\node() at (9, -2.9){$0$};
%	
%	\draw[decoration={brace,raise=5pt}, decorate, line width=0.25mm] (10.5, 3) -- node[right=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{a}{2} \pm c_1\sqrt{a}}$} (10.5, 2);
%	
%	%%%%%%%%%%%%%%%%%%%% EXTRA GOODIES %%%%%%%%%%%%%%%%
%	
%	\draw[-latex] (2.35, 0.1) -- (4.5, 2.25);
%	\draw[-latex] (2.35, 0.1) -- (4.5, -2.25);
%	\node () at (2.35, 0.1) [circle,fill,inner sep=1pt]{};
%	
%	\node (control) at (0, -4.75){$\zo^{\bC} \equiv \zo^m$};
%	\node (action) at (9, -4.75){$\zo^{\bA} \equiv \zo^{a}$};
%	
%\end{tikzpicture}
%
%\caption*{A draw of $\fno\sim\Dno$.} 
%%\red{{\bf Rocco:} I think given the previous caption we can omit everything but the preceding sentence from this caption? Also, can we get both pictures on the same page? (The pictures look great!)}
%% As before, the left hand side depicts the control subcube with the terms of the Talagrand DNF, and the right hand side depicts the action subcube. The cross-hatched region in the control subcube corresponds to outcomes of the control bits for which the action subcube determines the value of $\fno$, and the dashed lines indicate Hamming levels.}
%%}
%\label{fig:montone-yes}
%	
%\end{figure}
%
%


==> sections/intersectingness.tex <==
%!TEX root = ../tolerant.tex


\def\Dy{\Dyes}
\def\Dn{\Dno}
\def\prob{\textrm{Pr}}
\def\ManyOne{\textsf{ManyOne}}
\def\GoodTalagrand{\textsf{GoodTalagrand}}
\def\Bad{\textsf{Bad}}

\section{Lower Bounds for Testing Intersecting Families}
\label{sec:intersecting}

We start with some objects that we need in the construction of the two distributions $\Dyes$ and $\Dno$.\xnote{We used Dyes and Dno in preliminaries. {\bf Rocco:} I switched to $\Dyes$ and $\Dno$, let me know if I missed any}

We partition the variables $x_1,\cdots,x_n$ into \emph{control} variables and \emph{action} variables as follows: Let $a\coloneqq \sqrt{n}/\eps$ and ${A}\subseteq [n]$ be a fixed subset of $[n]$ of size $a$. Let $C\coloneqq [n]\setminus A$. We refer to the variables $x_i$ for $i\in C$ as \emph{control variables} and the variables $x_i$ for $i\in A$ as \emph{action variables}. We first define two pairs of functions over $\{0,1\}^A$ on the action variables as follows (we will use these functions later in the definition of $\Dy$ and $\Dn$):

\begin{equation*}
g^{(+,0)}(x_A) =
	\begin{cases}
       \ 0 & |x_A|>\frac{a}{2}+\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-\sqrt{a},\frac{a}{2}+\sqrt{a}]; \\[0.5ex]
       \ 0 & |x_A|<\frac{a}{2}-\sqrt{a}.
    \end{cases}
\quad g^{(+,1)}(x_A) =
	\begin{cases}
       \ 1 & |x_A|>\frac{a}{2}+\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-\sqrt{a},\frac{a}{2}+\sqrt{a}]; \\[0.5ex]
       \ 1 & |x_A|<\frac{a}{2}-\sqrt{a}.
    \end{cases}
\end{equation*}
and
\begin{equation*}
g^{(-,0)}(x_A) =
	\begin{cases}
       \ 1 & |x_A|>\frac{a}{2}+\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-\sqrt{a},\frac{a}{2}+\sqrt{a}]; \\[0.5ex]
       \ 0 & |x_A|<\frac{a}{2}-\sqrt{a}.
    \end{cases}
\quad g^{(-,1)}(x_A) =
	\begin{cases}
       \ 0 & |x_A|>\frac{a}{2}+\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-\sqrt{a},\frac{a}{2}+\sqrt{a}]; \\[0.5ex]
       \ 1 & |x_A|<\frac{a}{2}-\sqrt{a}.
    \end{cases}
\end{equation*}

Now we are ready to define the distributions $\Dy$ and $\Dn$ over $f:\{0,1\}^{n+2}\rightarrow\{0,1\}$. We follow the convention that random variables are in boldface and fixed quantities are in the standard typeface.




%have two random functions $\bm{g}_i,\tilde{\bm{g}}_i:\{0,1\}^a\rightarrow \{0,1\}$ (the distribution of them will be clear after we specify which of $\Dy$ and $\Dn$ we are working on).

%Given $\bm{A}$, $\bT$ and $\bb$,
A function $\bm{f}^+\sim \Dy$ is drawn as follows.
We start by sampling a subset $\bm{A}\subseteq [n]$ of size $a$ uniformly at random and let $\bm{C}\coloneqq [n]\setminus \bm{A}$. Note that there are in total $n-a$ control variables. We let $L\coloneqq 0.1\cdot2^{\sqrt{n-a}/\epsilon}$ and draw an $L$-term monotone Talagrand DNF $\bm{T}\sim \Tal(n-a,\eps)$ on $\bm{C}$ as described in \Cref{def:talagrand}. Finally, we sample $L$ random bits $\bm{b}\in\{0,1\}^L$ uniformly at random. 
Given $\bA,\bT$ and $\bb$, $\bm{f}^+$ is defined %by sampling $\bm{A}\subseteq [n]$ (and $\bm{C}\coloneqq [n]\setminus \bm{A}$), the Talagrand terms $\bm{T}$, and the random bits $\bm{b}\in\{0,1\}^L$ and 
  by letting  $\bm{f}(x,0,0)=\bm{f}(x,1,1)=0$ for all $x\in\{0,1\}^n$, and letting

\begin{align*}
\bm{f}^+(x,0,1) &=
	\begin{cases}
       \ 0 & |S_{\bm{T}}(x_{\bm{C}})|\neq 1; \\[0.5ex]
       \ g^{(+,0)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=0; \\[0.5ex]
       \ g^{(+,1)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=1.
    \end{cases}\\[1ex]
 \bm{f}^+(x,1,0) &=
	\begin{cases}
       \ 0 & |S_{\bm{T}}(\overline{x}_{\bm{C}})|\neq 1; \\[0.5ex]
       \ \red{g^{(+,1)}}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=0; \\[0.5ex]
       \ \red{g^{(+,0)}}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=1
    \end{cases}
\end{align*}
\rnote{Do we want to swap the two red entries above? Right now it is not consistent with the $\bm{f}^-$ definition (and it seems more natural to have $g^{(+,1)}$ when $\bm{b}_\ell$ is $1$ than when it is 0)}
(recall that $\overline{x}$ is the bitwise complement of string $x$).

To draw a function $\bm{f}^-\sim \Dy$, we sample $\bA,\bT$ and $\bb$ exactly as in the definition of $\Dy$ above, and we replace $g^{(+,0/1)}$ by $g^{(-,0/1)}$ in the construction described above. In more detail, $\bm{f}^-$ is defined by 
%For the functions in $\Dn$, we will replace $g^{(+,0/1)}$ and by $g^{(-,0/1)}$. In particular, $f^-\sim \Dn$ is defined by sampling $\bm{A}\subseteq [n]$ (and $\bm{C}\coloneqq [n]\setminus \bm{A}$), the Talagrand terms $\bm{T}$, and the random bits $\bm{b}\in\{0,1\}^L$ and letting  
  $\bm{f}(x,0,0)=\bm{f}(x,1,1)=0$ for all $x\in\{0,1\}^n$, and  
\begin{align*}
\bm{f}^-(x,0,1) &=
	\begin{cases}
       \ 0 & |S_{\bm{T}}(x_{\bm{C}})|\neq 1; \\[0.5ex]
       \ g^{(-,0)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=0;\\[0.5ex]
       \ g^{(-,1)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=1.
    \end{cases}\\
\bm{f}^-(x,1,0) &=
	\begin{cases}
       \ 0 & |S_{\bm{T}}(\overline{x}_{\bm{C}})|\neq 1; \\[0.5ex]
       \ g^{(-,0)}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=0; \\[0.5ex]
       \ g^{(-,1)}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=1.
    \end{cases}
\end{align*}
\rnote{Let's add a diagram for the overall construction - I think Shivam said he's working on this?  I think we also need to acknowledge that this is a variant of the PRW construction - we can do that either here or in the techniques section in the introduction (or in both places). Maybe it is better to do it there - I'll put this into that section.}



\subsection{Distance to Intersectingness}

\rnote{I think we will get rid of some but not all of this section; in particular we reference \Cref{lem:hehe2} later (though I think we will want to change the exact statement since we don't care about intersectingness now). I colored gray parts that I think we may not need, but I might be wrong}

\gray{
In this section, we will analyze the distance to intersectingness of functions in the support of $\Dy$ and $\Dn$.

\begin{lemma}
	Every function $f^+$ in the support of $\Dy$ is intersecting.
\end{lemma}
\begin{proof}
	Consider any function $f^+$ in the support of $\Dy$ and any two points $u,v\in\{0,1\}^{n+2}$ such that $f(u)=f(v)=1$. We will show that there exists $i\in[n+2]$ such that $u_i=v_i=1$.
	
	Since $f(u)=f(v)=1$, we have $u_{n+1}\neq u_{n+2}$ and $v_{n+1}\neq v_{n+2}$. If the last two bits of $u$ are the same as the last two bits of $v$ then  we are done, so without loss of generality assume that $u=(x,0,1)$ and $v=(y,1,0)$ where $x,y\in\{0,1\}^n$. Then by definition of $f^+$ we must have that $|S_T(x_C)|=1$ and $|S_T(\overline{y}_C)|=1$.
	
	Let $S_T(x_C)=\{\ell\}$. We will show that $S_T(\overline{y}_C)\neq\{\ell\}$, which implies that $y_i=1$ for some $i\in T_{\ell}$, and hence  $x_i=y_i=1$ for that value of $i$. We show the contrapositive. If  $S_T(\overline{y}_C)=\{\ell\}$ as well, then we have $f(x,0,1)=g^{(+,b_{\ell})}(x_A)$ and $f(y,1,0)=g^{(+,\overline{b_{\ell}})}(y_A)$. But since $f(x,0,1)=1$, we have $b_{\ell}=1$. Since $g^{(+,0)}$ is constantly zero, we have $f(y,1,0)=g^{(+,\overline{b_{\ell}})}(y_A)=0$, leading to a contradiction.
	
	This finishes the proof.
\end{proof}
}
\gray{
We include the characterization of the distance to intersectingness.


\begin{lemma} \label{lem:dist-to-intersecting}
	Given a boolean function $f:\{0,1\}^n\rightarrow\{0,1\}$, we have 
		$$\dint(f)=|M|/2^n,$$
	where $M$ is a maximum sized set of disjoint \textsf{I}-violating pairs of $f$.
\end{lemma}
\begin{proof}
	Let $M=\{(x^1,y^1),\cdots,(x^{|M|},y^{|M|})\}$ be the maximum sized set of disjoint \textsf{I}-violating pairs of $f$.
	
	Observe that any intersecting function $g$ must satisfy $g(x^i)=0$ or $g(y^i)=0$ for all $1\leq i\leq |M|$. This means the distance between $f$ and $g$ is at least $M/2^n$, so $\dint(f)\geq |M|/2^n$.
	
	For the other direction, we show that the function $g$ defined below satisfies that $g$ is intersecting and $\dist(f,g)=|M|/2^n$ (so $\dint(f) \leq |M|/2^n$)
	
\begin{equation*}
g(x) =
	\begin{cases}
       \ 0 & x=x^i\text{ for some }1\leq i\leq |M|; \\[0.5ex]
       \ f(x) & \text{otherwise}.
    \end{cases}
\end{equation*}
It is clear that $\dist(f,g)=|M|/2^n$. To see that $g$ is intersecting, suppose that there are $x,y$ such that $g(x)=g(y)=1$ and $x\cap y=\varnothing$. Then it must be the case that\rnote{Sorry for being dense; I see that $x$ and $y$ can't belong to $\{x^1,\cdots,x^{|M|}\}$ but why is it the case that they cannot belong to $\{y^1,\cdots,y^{|M|}$? If we set $g$ to 0 on the points $y^i$ as well then I see why this would be true; I think this would also give us the $1/2$ which may be missing from the RHS of the statement. Sorry if I'm misunderstanding something here.} $x,y\not\in\{x^1,\cdots,x^{|M|},y^1,\cdots,y^{|M|}\}$, so $f(x)=g(x)=1$ and $f(y)=g(y)=1$, which violates the assumption that $M$ is maximal.
\end{proof}
}

We next show that $\bm{f}^-\sim \Dn$ is $\Omega(\eps)$-far from intersecting with high probability.

\begin{lemma}\label{lem:hehe2}
	$\Pr_{\bm{f}^-\sim \Dn}[\bm{f}^-\text{ is } \Omega(\eps)\text{-far from intersecting}]\geq 0.75$.
%	Every function $f^-$ in the support of $\hat{\calD}^-$ is $\Omega(\eps)$-far from intersecting.
\end{lemma}
\begin{proof}	
\red{For conciseness we write $n'$ to denote $n-a$ throughout this proof.}
We first introduce the event $\GoodTalagrand(T)$, which states that there exists an $\Omega(\eps)$-fraction of points $x \in \{0,1\}^{\red{n'}}$ such that $|S_T(x)|=1$. 
Formally, let $t\cdot \eps$ be the number of $x$ in $\{0,1\}^{\red{n'}}$ such that\rnote{Minor note: we were a little inconsistent here and elsewhere about whether to denote the number of 1's in a string $x$ as $\|x\|_1$ or just $|x|$. Since we talk about how we view strings and subsets interchangeably, I went with $|x|$ here - let's check to make sure we are consistent throughout?} $|x| \in [\red{n'}/2, \red{n'}/2 + 0.05\eps\sqrt{\red{n'}}]$ and let $\GoodTalagrand(T)$ be the event that $\mathbb{E}_{|\bm{x}|\in[\red{n'}/2, \red{n'}/2 + 0.05\eps\sqrt{\red{n'}}]}\left[\textbf{1}_{\{|S_T(x)|=1\}}\right]\geq t\cdot \eps/100$. We will show that $\prob_{\bm{T}\sim\Tal(\red{n'},\eps)}[\GoodTalagrand(\bm{T})]\geq 0.76$.

Let $p$ denote $\prob_{\bm{T}\sim\Tal(\red{n'},\eps)}[\GoodTalagrand(\bm{T})]$. \blue{
Recall that in \Cref{prop:talagrand-unique-property}, we have shown that $\Prx_{\bm{T}}\sbra{|S_{\bm{T}}(x)| = 1} \geq 0.8$  for any $x\in\{0,1\}^{\red{n'}}$ with $|x|_1 \in [\red{n'}/2, \red{n'}/2 + 0.05\eps\sqrt{\red{n'}}]$.}\rnote{Right now I think \Cref{prop:talagrand-unique-property} only gives us that the probability is at least $0.03$, not $0.8$. Do we want to change parameters in \Cref{prop:talagrand-unique-property} so we get $0.8$, or change the argument here?} So we have $$p\cdot t\eps+(1-p)\cdot t\eps/100\geq t\eps\Prx_{\bm{T}}\sbra{|S_{\bm{T}}(x)| = 1} \geq 0.8t\eps,$$ 
which implies that $p\geq 79/99> 0.76.$

Fix an arbitrary $T$ in the support of $\Tal(\red{n'},\eps)$ such that $\GoodTalagrand(T)$ happens. Note that for each $x$ such that $S_T(x)=\{\ell\}$ for some $\ell\in[L]$, $\mathbb{E}[\bm{b}_{\ell}]=1/2.$ So by  linearity of expectation and Markov's inequality, we know that with probability at least $99\%$, there is an $\Omega(\eps)$-fraction of points $x$ such that $S_T(x)=\{\ell\}$ and $b_{\ell}=1$. We write $\ManyOne$ to denote this event.

Assuming that both $\ManyOne$ and $\GoodTalagrand$ happen (whose probability is at least $75\%$), below we will show that $f^-$ is $\Omega(\eps)$-far from intersecting, which will finish the proof.

For each $x_C\in\{0,1\}^{\red{n'}}=\{0,1\}^{n-a}$ with $S_T(x_C)=\{\ell\}$ and $b_{\ell}=1$, we show that there is a set of violating pairs of size at least $\Omega(2^a)$. In particular, we  show that there are at least $\Omega(2^a)$ pairs $(x^i_A,y^i_A)$ such that $f(x_C,x^i_A,0,1)=f(\overline{x}_C,y^i_A,1,0)=1$ but $x^i_A\cap y^i_A=\varnothing$. 


To this end, we include a folklore claim and its proof for completeness.
\begin{claim}\label{claim: k regular graph bipartite matching}
	For integer $0\leq w\leq a$, let $P_w$ denote the set of points in $\{0,1\}^a$ with Hamming weight $w$, i.e.~$P_w = \{x\in\{0,1\}^a \ : \ |x|_1=w\}$. Then for any $0\leq w\leq a/2$, the bipartite graph $(P_w,P_{a-w})$ with the poset relations as edges has a perfect matching.
\end{claim}
\begin{proof}

	The key point is that $(P_w,P_{a-w})$ is a $k$-regular bipartite graph, where $k={a-w \choose w}$.
	
	 We apply Hall's theorem to show this claim. Consider any subset $S\subseteq P_{a-w}$. The number of edges associated with $S$ is exactly $k|S|$. Let $\calN(S)$ be the neighborhood of $S$. Then we know the number of edges associated with $\calN(S)$ is exactly $k|\calN(S)|$, and these edges include the $k|S|$ edges above. So we have $k|S|\leq k|\calN(S)|$, which means $|S|\leq |\calN(S)|$.
\end{proof}

Fix any point $x_C\in\{0,1\}^{\red{n'}}=\{0,1\}^{n-a}$ such that $S_T(x_C)=\{\ell\}$ and $b_{\ell}=1$ for some $\ell\in[L]$. Consider the action cube $\{0,1\}^a$. For any Hamming weight $w<\frac{a}{2}-\sqrt{a}$, fix a perfect matching $\{(x^i_A,\overline{y}^i_A)\}$ of $(P_w,P_{a-w})$. Then we note that $f(x_C,x^i_A,0,1)=1$, whereas $f(\overline{x}_C,y^i_A,1,0)=1$. The number of points with Hamming weight less than $\frac{a}{2}-\sqrt{a}$ is $\Omega(2^a)$, so there are $\Omega(2^a)$ violating pairs.

Then the lemma follows from the fact there are $\Omega(\eps\cdot 2^{n-a})$ points $x_C\in\{0,1\}^{n-a}$ such that $S_T(x_C)=\{\ell\}$ and $b_{\ell}=1$ for some $\ell\in[L]$ (since we assumed that both $\ManyOne$ and $\GoodTalagrand$ happen). So overall we have $\Omega(\eps\cdot 2^n)$ violating pairs, which means the function $f^-$ is $\Omega(\eps)$-far from intersecting.
\end{proof}

\subsection{Indistinguishability of $\Dy$ and $\Dn$}\label{sec:hehe1}

In this section we establish the indistinguishability of the distributions $\Dy$ and $\Dn$. Specifically, for any nonadaptive deterministic algorithm $\calA$ with query complexity $q=2^{0.1n^{1/4}/\sqrt{\eps}}$, we show that
\begin{equation} \label{eq:goal}
\Pr_{\bm{f}^+\sim \Dy}[\calA \text{ accepts }\bm{f}^+]\leq \Pr_{\bm{f}^-\sim \Dn}[\calA \text{ accepts }\bm{f}^-]+ 0.1.
\end{equation}

We begin with some simplifying assumptions: for any point $u\in\{0,1\}^{n+2}$ that is queried by the algorithm $\calA$ we assume that $u_{n+1}\neq u_{n+2}$ (since otherwise the answer to the query must be 0), and we assume that for each point $u \in \zo^{n+2}$ that is queried by ${\cal A}$ the point $\overline{u}$ is also queried as well (since this only affects the query complexity by at most a factor of two). So the set of $q$ query points of $\calA$ can be  characterized by a set $Q_{\calA}\coloneqq \{x^1,\cdots,x^q\}\subseteq \{0,1\}^n$, where both $(x^i,0,1)$ and $(\overline{x}^i,1,0)$ are queried for each $i\in[q]$.

A crucial step of the argument is that the only way for $\calA$ to distinguish $\Dy$ and $\Dn$ is to query two points $x^i,x^j$ with $S_T(x^i_C)=S_T(x^j_C)=\{\ell\}$ for some $\ell \in [L]$ such that one is in the top region and the other is in the bottom region of the action cube, namely $|x^i_A|>\frac{a}{2}+\sqrt{a}$ and $|x^j_A|<\frac{a}{2}-\sqrt{a}$. We let $\Bad$ denote this event (that $Q_{\calA}$ contains two points $x^i,x^j$ satisfying the above conditions).

Formally, the following claim asserts that conditioned on $\Bad$ not happening, the distributions $\mathrm{view}_{\calA}(\Dy|_{\overline{\Bad}})$ and $\mathrm{view}_{\calA}(\Dn|_{\overline{\Bad}})$ are identical.


\begin{lemma}\label{lemma: Bad is the only different place between Dy and Dn}
	$\mathrm{view}_{\calA}(\Dy|_{\overline{\Bad}})=\mathrm{view}_{\calA}(\Dn|_{\overline{\Bad}}).$
\end{lemma}
\begin{proof}
	The distributions of the partition of $[n]$ into control variables $\bm{C}$ and action variables $\bm{A}$ are identical for $\Dy$ and $\Dn$. So fix an arbitrary partition $C$ and $A$.
	
	We divide the points $Q_{\calA}$ into disjoint groups according to $x_C$. More precisely, for every $\ell\in [L]$, let $Q_{\calA}(\ell)=\{x^i\mid S_T(x^i_C)=\{\ell\}\}$. Let $\bm{f}_{\ell}(x,0,1)$ denote the function $\bm{f}(x,0,1)$ restricted to inputs $x\in Q_{\calA}(\ell)$, and let $\bm{f}_{\ell}(\overline{x},1,0)$ similarly denote the function $\bm{f}(\overline{x},1,0)$ restricted to inputs $x\in Q_{\calA}(\ell)$. Note that for a fixed $\ell\in[L]$, the functions $\bm{f}_{\ell}(x,0,1)$ and $\bm{f}_{\ell}(\overline{x},1,0)$ only depend on the random bit $\bm{b}_{\ell}$. As a result, the distributions of functions $\bm{f}_{\ell}(x,0,1)$ and $\bm{f}_{\ell}(\overline{x},1,0)$ for different $\ell$ are independent.
	
	So fix an arbitrary $\ell\in[L]$. The condition that $\Bad$ does not happen implies that $\bm{f}_{\ell}(x^i,0,1)=\bm{f}_{\ell}(x^j,0,1)$ for all $x^i,x^j\in Q_{\calA}(\ell)$, which holds for both $\Dy$ and $\Dn$. Note also that $\bm{f}_{\ell}(\overline{x}^i,1,0)=1-\bm{f}_{\ell}(x^i,0,1)$ also holds for both $\Dy$ and $\Dn$. 
	
	So it suffices for us to show that the distributions of $\bm{f}_{\ell}(x^i,0,1)$ are the same for $\Dy$ and $\Dn$. To see this, we note that $\bm{b}_i$ is an independent uniform random bit, so $\bm{f}_{\ell}(x^i,0,1)=0$ with probability $1/2$ and $\bm{f}_{\ell}(x^i,0,1)=1$ with probability $1/2$, which holds for both $\Dy$ and $\Dn$.
	
	This finishes the proof.
\end{proof}

Next, we show that the probability that $\Bad$ happens is small
(recall that $q=2^{0.1n^{1/4}/\sqrt{\eps}}$):

\begin{lemma}\label{lemma: Bad is unlikely}
	For any set of points $Q_{\calA}=\{x^1,\cdots,x^q\}\subseteq \{0,1\}^n$, $\prob[\Bad]=o(1)$.
\end{lemma}
\begin{proof}
	Fix any two points $x,y\in\{0,1\}^n$. We will upper bound the probability that $S_{\bT}(x_{\bm{C}})=S_{\bT}(y_{\bm{C}})=\{\ell\}$ for some $\ell\in[L]$ and $|x_{\bm{A}}|<\frac{a}{2}-\sqrt{a}$ and $|y_{\bm{A}}|>\frac{a}{2}+\sqrt{a}$. Call this specific event $\Bad_{xy}$.
	
	Let $I_{01}$ be the set of indices $i$ such that $x_i=0$ and $y_i=1$. On the one hand, to have $\Bad_{xy}$ happen, we must have that ($\diamond$) $|I_{01}\cap \bm{A}|\geq 2\sqrt{a}$. On the other hand, to have  $S_{\bT}(x_{\bm{C}})=S_{\bT}(y_{\bm{C}})=\{\ell\}$, we must have that 
	%\gray{($\star$) $I_{01}\cap \bm{C}$ can not contain any index of $\bm{T}_{\ell}$.} \rnote{The condition $\star$ is actually a condition about all $\ell=1,2,\dots,L$, right - there is no fixed value of $\ell$ at this point in the argument, is that correct? Maybe we should rewrite the definition of $\star$ slightly? (Yuhao, this is connected to the question Shivam sent you a few days back - the answer you gave, which seems correct, is the blue stuff up above.) }
($\star$) there exists an $\ell \in [L]$ such that $S_{\bT}(x)=S_{\bT}(y)=\{\ell\}.$
So we have $\prob[\Bad_{xy}]\leq \min(\prob[\diamond],\prob[\star])$; we will show that
\[
\min(\prob[\diamond],\prob[\star])
\leq 2^{-n^{1/4}/\sqrt{\eps}}.
\]
	
	Let $t=|I_{01}|$. Then by the random choice of the coordinates defining the action cube $\bA$, we have
%	\[\prob[\diamond]\leq \prob\left [\mathrm{Bin}\left (t,\frac{a}{n}\right )\geq 2\sqrt{a}\right]\leq n\cdot {t\choose 2\sqrt{a}}\cdot \left(\frac{a}{n}\right)^{2\sqrt{a}}\leq n\cdot \left(\frac{et}{2\sqrt{a}}\right)^{2\sqrt{a}}\cdot \left(\frac{a}{n}\right)^{2\sqrt{a}}\leq n\cdot \left(\frac{et\sqrt{a}}{2n}\right)^{2\sqrt{a}}\]
\begin{align*}
    \prob[\diamond] & \leq \prob\left [\mathrm{Bin}\left (t,\frac{a}{n}\right )\geq 2\sqrt{a}\right]\leq n\cdot {t\choose 2\sqrt{a}}\cdot \left(\frac{a}{n}\right)^{2\sqrt{a}}\\
    & \leq n\cdot \left(\frac{et}{2\sqrt{a}}\right)^{2\sqrt{a}}\cdot \left(\frac{a}{n}\right)^{2\sqrt{a}}\leq n\cdot \left(\frac{et\sqrt{a}}{2n}\right)^{2\sqrt{a}}.
\end{align*}
%\gray{and
%\begin{align*}
%    \prob[\star] & \leq \left(1-\frac{t}{n-a}\right)^{\sqrt{n-a}/\eps}\leq e^{-t/(\eps\sqrt{n-a})}\leq e^{-t/(\eps\sqrt{n})}.
%\end{align*}
%}
To bound $\prob[\star]$, we use
\begin{align*}
\prob[\star]&=\prob[S_{\bT}(x)=S_{\bT}(y) \ \& \ \exists \ell \in [L] \text{~such that~}S_{\bT}(y)=\{\ell\}]\\
&\leq \prob[S_{\bT}(x)=S_{\bT}(y) \ \mid \ \exists \ell \in [L] \text{~such that~}S_{\bT}(y)=\{\ell\}]\\
&\leq \max_{\ell \in [L]} \prob[S_{\bT}(x)=S_{\bT}(y) \ \mid \ S_{\bT}(y)=\{\ell\}]\\
&\leq \left(1-\frac{t}{n-a}\right)^{\sqrt{n-a}/\eps}\leq e^{-t/(\eps\sqrt{n-a})}\leq e^{-t/(\eps\sqrt{n})},
\end{align*}
where the last line above is by the definition of the random process $\bT \sim \Tal(\red{n'},\eps)$.

When $t\leq \frac{1}{4}n^{3/4}/\sqrt{\eps}$, we have $\prob[\diamond]\leq 2^{-n^{1/4}/\sqrt{\eps}}.$ When $t\geq \frac{1}{4}n^{3/4}/\sqrt{\eps}$, we have $\prob[\star]\leq 2^{-0.25n^{1/4}/\sqrt{\eps}}.$

	
	So overall we have $$\prob[\Bad_{xy}]\leq \min(\prob[\diamond],\prob[\star])\leq 2^{-0.25n^{1/4}/\sqrt{\eps}}.$$
	
	By a union bound for all pairs of points of $Q_{\calA}$, we know that $$\prob[\Bad]\leq 2^{-0.25n^{1/4}/\sqrt{\eps}}\cdot \left(2^{0.1n^{1/4}/\sqrt{\eps}}\right)^2=o(1),$$
	and the lemma is proved.
\end{proof}


Now we are ready to prove Theorem~\ref{thm:main-lb-intersecting}.

\begin{proof}[Proof of Theorem~\ref{thm:main-lb-intersecting}]

\begin{align*}
    &\quad \Pr_{\bm{f}^-\sim \Dn}[\calA \text{ accepts }\bm{f}^-]-\Pr_{\bm{f}^+\sim \Dy}[\calA \text{ accepts }\bm{f}^+]\\
    &= \Pr[\Bad]\cdot \left(\Pr_{\bm{f}^-\sim \Dn|_{\Bad}}[\calA \text{ accepts }\bm{f}^-]-\Pr_{\bm{f}^+\sim \Dy|_{\Bad}}[\calA \text{ accepts }\bm{f}^+]\right)\\
    & \leq \Pr[\Bad]\leq o_n(1),
\end{align*}
where the first equality follows from Lemma~\ref{lemma: Bad is the only different place between Dy and Dn}. 


Theorem~\ref{thm:main-lb-intersecting} follows from Yao's minimax principle (\Cref{thm:yao-minimax}) \gray{by taking the distribution as $\frac{1}{2}(\Dy+\Dn)$}.\rnote{Minor quibble: the way \Cref{thm:yao-minimax} is stated I think we don't need to mention $\frac{1}{2}(\Dy+\Dn)$; shall we just take out the gray phrase?}
\end{proof}



==> sections/scratchspace.tex <==
\section{Scratchspace}

\snote{TODO: Sometimes we have $\bT$ and sometimes $\bm{T}$---have to align throughout.}


\input{images/monotone-y}
\input{images/monotone-n}
\input{images/junta}

\subsection{Optimality of the Talagrand DNF on the Control Subcube}







==> sections/tolerant-xi-conflicted-copy.tex <==
%!TEX root = ../int-uc-tolerant.tex

\section{Lower Bounds for Tolerant Testing}
\label{sec:tolerant}

\def\Talt{{\Tal}^*}
\def\nil{\textsf{nil}}

\subsection{Construction of $\Dy$ and $\Dn$ for Monotonicity and Unateness}

The construction of the pair of distribution $\Dy$ and $\Dn$ is similar to 
  the construction in Section \ref{}.
Let $\epsilon\in (0,1)$ be a parameter with $\epsilon\ge c_0/\sqrt{n}$ for some sufficiently 
  large constant $c_0$.
Let $a=\sqrt{n}/\epsilon$ and let $A\subset [n]$ be a subset of size $a$.
We start with a small modification on the four functions $g^{(+,0)},g^{(+,1)},g^{(-.0)},g^{(-,1)}$ by
  making the middle layers a bit narrower.
Let $h^{(+,0)},h^{(+,1)},h^{(-,0)}$ and $h^{(-,1)}$ be Boolean functions over $\{0,1\}^A$ defined as follows:
\begin{equation*}
g^{(+,0)}(x_A) =
	\begin{cases}
       \ 0 & |x_A|>\frac{a}{2}+c_1\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-c_1\sqrt{a},\frac{a}{2}+c_1\sqrt{a}]; \\[0.5ex]
       \ 0 & |x_A|<\frac{a}{2}-c_1\sqrt{a}.
    \end{cases}
\quad g^{(+,1)}(x_A) =
	\begin{cases}
       \ 1 & |x_A|>\frac{a}{2}+c_1\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-\sqrt{a},c_1\frac{a}{2}+c_1\sqrt{a}]; \\[0.5ex]
       \ 1 & |x_A|<\frac{a}{2}-c_1\sqrt{a}.
    \end{cases}
\end{equation*}
and
\begin{equation*}
g^{(-,0)}(x_A) =
	\begin{cases}
       \ 1 & |x_A|>\frac{a}{2}+c_1\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-c_1\sqrt{a},\frac{a}{2}+c_1\sqrt{a}]; \\[0.5ex]
       \ 0 & |x_A|<\frac{a}{2}-c_1\sqrt{a}.
    \end{cases}
\quad g^{(-,1)}(x_A) =
	\begin{cases}
       \ 0 & |x_A|>\frac{a}{2}+c_1\sqrt{a}; \\[0.5ex]
       \ 0 & |x_A|\in[\frac{a}{2}-c_1\sqrt{a},\frac{a}{2}+c_1\sqrt{a}]; \\[0.5ex]
       \ 1 & |x_A|<\frac{a}{2}-c_1\sqrt{a}
    \end{cases}
\end{equation*}
for some sufficiently small constant $c_1$ to be specified later.

%\begin{definition}[Talagrand's random DNF with Truncations] \label{def:talagrandtruncation}
%	\xnote{Should we add Let $\eps\in (0,1)$ here?}Let $L\coloneqq 0.1\cdot2^{\sqrt{n}/\epsilon}$. Let %\xnote{It seems that we used $\Talt$ for both the distribution of the sequence of terms and the distribution of functions.}$\Talt(n, \epsilon)$ be the distribution on $L$ terms obtained by drawing $L$ sets $\bT_1, \ldots, \bT_{L} \sse [n]$ where each set $\bT_i$ is obtained by drawing $\sqrt{n}/\eps$ elements of $[n]$ independently and with replacement. We use $\bm{T}$ to denote $\{\bm{T}_1,\cdots,\bm{T}_L\}$\xnote{Maybe it is easier to take $\bm{T}$ as an ordered tuple $(\bm{T}_1,\ldots,\bm{T}_L)$?}.
%		Then the Talagrand's DNF is given by
%		\[\boldf(x) = \bigvee_{\ell=1}^{L} \pbra{\bigwedge_{j\in \bT_{\ell}} x_{j}}\]
%when $\|x\|_1\in [n/2, n/2 + 0.05\epsilon\sqrt{n}]$; $\boldf(x)=0$ when $\|x\|_1<n/2$ and 
%  $\boldf(x)=1$ when $\|x\|_1>n/2+0.05\epsilon\sqrt{n}$.
%\end{definition}

\xnote{Have we defined the tolerant testing model?}
Let $m=n-a$.
We now describe the pair of distributions $\Dy$ and $\Dn$ over Boolean functions over $\{0,1\}^n$.
A function $\bm{f}^+\sim \Dy$ is drawn as follows.
We start by sampling $\bm{A}, \bm{T}$ and $\bm{b}$ in exactly the same way
  how they are sampled in Section \ref{}.
%a subset $\bm{A}\subseteq [n]$ of size $a$ uniformly at random and let $\bm{C}\coloneqq [n]\setminus \bm{A}$. Note that there are in total $n-a$ control variables. We let $L\coloneqq 0.1\cdot2^{\sqrt{n-a}/\epsilon}$ and draw a Talagrand DNF $\bm{T}\sim \Tal(n-a,\eps)$ on $\bm{C}$. Finally, we sample $L$ random bits $\bm{b}\in\{0,1\}^L$ uniformly at random. 
Given $\bA,\bT$ and $\bb$, $\bm{f}^+$ is defined %by sampling $\bm{A}\subseteq [n]$ (and $\bm{C}\coloneqq [n]\setminus \bm{A}$), the Talagrand terms $\bm{T}$, and the random bits $\bm{b}\in\{0,1\}^L$ and 
  by letting  %$\bm{f}(x,0,0)=\bm{f}(x,1,1)=0$ for all $x\in\{0,1\}^n$, and 
%\rnote{I think we're going to $S_f$ notation below}
\begin{align*}
\bm{f}^+(x ) &=
	\begin{cases}
       \ 1 & |S_{\bm{T}}(x_{\bm{C}})|>1\ \text{or}\ \|x_{\bm{C}}\|_1> m/2+0.05\epsilon\sqrt{m}; \\[0.5ex]
       \ 0 & |S_{\bm{T}}(x_{\bm{C}})|=0\ \text{or}\ \|x_{\bm{C}}\|_1<m/2 ; \\[0.5ex]
       \ h^{(+,0)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\},\ 
       \|x_{\bm{C}}\|_1\in [m/2,m/2+0.05\epsilon\sqrt{m}] \text{ and } \bm{b}_{\ell}=0; \\[0.5ex]
       \ h^{(+,1)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\},\ 
       \|x_{\bm{C}}\|_1\in [m/2,m/2+0.05\epsilon\sqrt{m}] \text{ and } \bm{b}_{\ell}=1.
    \end{cases}%\\[1ex]
% \bm{f}^+(x,1,0) &=
%	\begin{cases}
%       \ 0 & |S_{\bm{T}}(\overline{x}_{\bm{C}})|\neq 1; \\[0.5ex]
%       \ g^{(+,1)}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=0; \\[0.5ex]
%       \ g^{(+,0)}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=1.
 %   \end{cases}
\end{align*}

On the other hand, to draw a function $\bm{f}^-\sim \Dy$, we sample $\bA,\bT$ and $\bb$ in the exactly same way
  as in the definition of $\Dy$ above.
Replacing $g^{(+,0/1)}$ by $g^{(-,0/1)}$, $\bm{f}^-$ is defined by letting 
%For the functions in $\Dn$, we will replace $g^{(+,0/1)}$ and by $g^{(-,0/1)}$. In particular, $f^-\sim \Dn$ is defined by sampling $\bm{A}\subseteq [n]$ (and $\bm{C}\coloneqq [n]\setminus \bm{A}$), the Talagrand terms $\bm{T}$, and the random bits $\bm{b}\in\{0,1\}^L$ and letting  
%  $\bm{f}(x,0,0)=\bm{f}(x,1,1)=0$ for all $x\in\{0,1\}^n$, and  
\begin{align*}
\bm{f}^-(x ) &=
	\begin{cases}
       \ 1 & |S_{\bm{T}}(x_{\bm{C}})|>1\ \text{or}\ \|x_{\bm{C}}\|_1> m/2+0.05\epsilon\sqrt{m}; \\[0.5ex]
       \ 0 & |S_{\bm{T}}(x_{\bm{C}})|=0\ \text{or}\ \|x_{\bm{C}}\|_1<m/2 ; \\[0.5ex]
       \ h^{(-,0)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\},\ 
       \|x_{\bm{C}}\|_1\in [m/2,m/2+0.05\epsilon\sqrt{m}] \text{ and } \bm{b}_{\ell}=0; \\[0.5ex]
       \ h^{(-,1)}(x_{\bm{A}}) & S_{\bm{T}}(x_{\bm{C}})=\{\ell\},\ 
       \|x_{\bm{C}}\|_1\in [m/2,m/2+0.05\epsilon\sqrt{m}] \text{ and } \bm{b}_{\ell}=1.
    \end{cases}
%\bm{f}^-(x,1,0) &=
%	\begin{cases}
%       \ 0 & |S_{\bm{T}}(\overline{x}_{\bm{C}})|\neq 1; \\[0.5ex]
%       \ g^{(-,0)}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=0; \\[0.5ex]
 %      \ g^{(-,1)}(x_{\bm{A}}) & S_{\bm{T}}(\overline{x}_{\bm{C}})=\{\ell\} \text{ and } \bm{b}_{\ell}=1.
%    \end{cases}
\end{align*}
It is easy to verify that every function in the support of $\Dy$ is close to monotone (and thus, unate):


\def\bC{\mathbf{C}}
\def\bT{\mathbf{T}}

\begin{lemma}
Every function in the support of $\Dy$ is $(0.1\eps c_1)$-close to monotonicity.
\end{lemma}
\begin{proof}
Let $f$ be a function in the support of $\Dy$ defined using $A,T$ and $b$.
Let $f'$ be the partial function obtained from $f$ by replacing $f(x)$ with $\nil$ for any 
  $x\in \{0,1\}^n$ that satisfies $S_T(x_C)=\{\ell\}$ for some $\ell$,
\begin{align}\label{eq:hehe1}
|x_C|\in \left[m/2.m/2+0.05\eps\sqrt{m}\right]
\quad\text{and}\quad
|x_A|\in \left[a/2-c_1\sqrt{a},a/2+c_1\sqrt{a}\right].
\end{align}
Note that the fraction of points erased is at most
$0.05\eps\cdot 2c_1\le 0.1\eps c_1$. It suffices to show that the 
  partial function $f'$ is monotone.
  
To prove this, it suffice to show that for any $x\prec y$, if $f(x)=1$ and $f(y)\ne \nil$ then $f(y)=1$.
The case when $x$ satisfies $|S_T(x_C)|>1$ or $\|x_C\|_1>m/2+0.05\eps\sqrt{m}$ is trivial. 
Otherwise, $x$ must satisfy  $S_T(x_C)=\{\ell\}$ for some $\ell$ and \Cref{eq:hehe1}, and $b_\ell=1$.
Given that $x\prec y$, we have either $|S_T(y_C)|>1$, in which case $f(y)=1$ and we are done,
  or $|x_C|>m/2+0.05\eps\sqrt{m}$ in which case $f(y)=1$ and we are also done,
  or $S_T(y_C)=\{\ell\}$ and $|y_C|>\in [m/2,m/2+0.05\eps\sqrt{m}]$.
For the latter, we have either $y_A$ is in the middle layers and $f(y)=\nil$ or $y_A$ is not 
  in the middle layers and thus, $f(y)=1$. This finishes the proof of the lemma.
\end{proof}

Some basic facts about middle layers of a hypercube:

\begin{fact}
Every integer $\ell\in [-0.1\sqrt{n},0.1\sqrt{n}]$ satsfies 
$$
\frac{1}{4\sqrt{n}}\le \frac{{n\choose n/2+\ell}}{2^n}\le \frac{1}{\sqrt{n}}
$$
\end{fact}

Next we show that with high probability, a function drawn from $\Dn$ is far from unate.

\begin{lemma}
With probability at least ?, $\bm{f}\sim \Dn$ is $\Omega(\eps)$-far from unate.
\end{lemma}
\begin{proof}
First it follows from the proof of \Cref{prop:talagrand-unique-property}
  that the expected fraction of $x\in \{0,1\}^\bC$ such that $|S_\bT(x )|=1$ and 
  $|x |\in \left[m/2,m/2+0.05\eps\sqrt{m}\right]$ is at least 
  $0.03\cdot 0.05\eps$
We will use the following claim:

\begin{claim}
Fix any set $A\subset [n]$ of size $a$.Z any $r\JKL
\/in \{0,1\}^A$, either $$g_0:= g^{(-,0)}(x\OID r)\quad\text{or}\quad 
g_1:=g^{(-,1)}(x\oplus r)$$ is $\Omega(1)$-far
  from monotone.
\end{claim}
\begin{proof}
Fix an $r\in \{0,1\}^A$.
Without loss of generality we assume that $r$ satisfies $|r|\le a/2$ with
  $r_1=\cdots=r_k=0$, where $k=a-|r|\ge a/2$,
  and show that $g_1$ is $\Omega(1)$-far from monotone.
To this end, it suffices to give $\Omega(2^n)$ many disjoint pairs $(x,y)$
  such that $x\prec y$, $g_1(x)=1$ and $g_1(y)=0$.
For this purpose, we pick any $z\in \{0,1\}^{a-k}$ such that $|z|\in [(a-k)/2-\sqrt{a-k},
(a-k)/2+\sqrt{a-k}]$. Note that the number of such $z$, by Fact ?, is at least $\Omega(2^{a-k})$.

On the other hand, for any fixed $z$, we create disjoint pairs $(x,y)$ such that 
  $x\prec y$, $x_{[k+1:a]}=y_{[k+1:a]}=z$\xnote{Not sure we have introduced the notation before.},
  $|x_{[k]}|\le k/2-22c_1\sqrt{a}$ and $|y_{[k]}|\ge k/2+2\sqrt{a}$
  so that we have $g_1(x)=1$ and $g_1(y)=0$.
It follows from ??? that the number of such pairs is
  at least $2^{k}/9$ when $c_1$ is chosen to be sufficiently small.
Therefore, the total number of disjoint pairs is at least
$$
\frac{4c_1}{9}\cdot 2^a.
$$
and the claim follows.
\end{proof}

To prove Lemma \ref{}, we have from ? and ? that with high probability over
  $\bA,\bT$ and $\bb$, the number of strings $y\in \{0,1\}^{\bC}$ that satisfies 
  $S_{\bT}(y)|=\{\ell\}$ for some $\ell$ and (in middle layers) and $\bb_\ell=1$
  is at least $\Omega(\eps)\cdot 2^{n-a}$ and the number of strings 
  $y\in \{0,1\}^{\bC}$ that satisfies 
  $S_{\bT}(y)|=\{\ell\}$ for some $\ell$ and (in middle layers) and $\bb_\ell=0$
  is also at least $\Omega(\eps)\cdot 2^{n-a}$.
The lemma then follows from Claim \ref{}.
\end{proof}

To summarize, we e

\subsection{Indistinguishability of $\Dy$ and $\Dn$}

\subsection{Construction of $\Dy$ and $\Dn$ for Monotonicity and Unateness}

\subsection{Indistinguishability of $\Dy$ and $\Dn$}

%\rnote{
%Monotonicity and juntas: computing the distance to mono / junta in yes- and no- cases for our construction, for a given value of $\eps$, and then pointing out that we get $(\eps_1,\eps_2)$-tolerant nonadaptive lower bounds for the resulting $\eps_1$ and $\eps_2$ values. The exciting setting is $\eps=$constant.
%Do we get unateness results as well?}

%\red{Xi has the token?}

==> sections/ubs.tex <==
%!TEX root = ../int-uc-tolerant.tex

\section{Upper Bounds}
\label{sec:ubs}

\subsection{Upper bound for testing union-closedness} 
In this section, first we will give some useful definitions in the context of union-closed functions. Subsequently, we will give a tester for union-closedness. 
\begin{definition}~\label{def:UC-violating}
For a function $f: \{0,1\}^n \rightarrow \{0,1\}$, a sequence  $(x_1, \ldots, x_k, x_1 \cup \ldots \cup x_k)$ (where each $x_i \in \{0,1\}^n$) is said to be a \emph{union-closed violating tuple} (written ``\textsf{UC}-violating tuple'' for short) if the following holds: for each $1 \le j \le k$, $f(x_j)=1$ and $f(x_1 \cup \ldots \cup x_k)=0$.


Furthermore, we say that two \textsf{UC}-violating tuples $(x_1, \ldots, x_k, x_1 \cup \ldots \cup x_k)$ and $(y_1, \ldots, y_k, y_1 \cup \ldots \cup y_k)$ are \rnote{Changed this from ``end-disjoint'' to ``end-distinct'' here and elsewhere - since we are viewing them as sets and the sets don't have to be disjoint, I think this may be a better term} {\em end-distinct} if $x_1 \cup \ldots \cup x_k \not = y_1 \cup \ldots \cup y_k$.  

Finally, we say that   a    \textsf{UC}-violating tuple $(x_1, \ldots, x_k, x_1 \cup \ldots \cup x_k)$ is \emph{minimal} if for any $1 \le j \le k$, it holds that $\cup_{i \not =j} x_i \subsetneq (x_1 \cup \ldots \cup x_k)$. 
\end{definition} 
%\begin{definition}~\label{def:UC-triple}
%\rnote{(minor) Maybe let's have this as a second sentence of the previous definition rather than a separate definition?}For a function $f: \{0,1\}^n \rightarrow \{0,1\}$, a triple $(x,y,z)$  (where $x, y, z \in \{0,1\}^n$) is said to be a \textsf{UC}-violating triple if the following holds:  $x \cup y = z$, $f(x)=1$, $f(y)=1$ and $f(z)=0$. 
%\end{definition} 


%\begin{definition}~\label{def:intersection-violating}
%For a function $f: \{0,1\}^n \rightarrow \{0,1\}$, a pair $(x,y)$ is said to be an \textsf{Int}-violating pair if $f(x) = f(y)=1$ and $x \cap y =\emptyset$. 
%\end{definition} 

Given $f: \zo^n \to \zo$, we write $\duc(f)$ to denote the distance from $f$ to the property which consists of all union-closed functions, i.e.~
\[
\duc(f) = \min_{g: \zo^n \to \zo \text{~is~union-closed}} \dist(f,g).
\]
The following lemma shows that any function which is far from union-closed must have many end-distinct violating tuples:
\begin{lemma}~\label{lem:distance-uc}
Suppose $f: \{0,1\}^n \rightarrow \{0,1\}$ is such that $\duc(f) > \epsilon$. Then, $f$ has at least $\epsilon \cdot 2^n$ many  end-distinct \textsf{UC}-violating
tuples 
 %\red{triples}.\rnote{I think ``triple'' here should be ``tuple'', right - we didn't say anything about triples so far?}
\end{lemma}

\anote{Can be simplified?}

\begin{proof}
For the function $f$, let ${\cal C}$ be a maximal collection of end-distinct $\mathsf{UC}$-violating tuple. Let ${\cal B}$ be the set of all the points in $\{0,1\}^n$ which appear as the last coordinate of a tuple in ${\cal C}$. Define ${\cal A} =\{0,1\}^n \setminus {\cal B}$.


We now define $\tilde{f}: \{0,1\}^n \rightarrow \{0,1\}$ as follows: 
\begin{enumerate}
\item $\tilde{f}(x)=1$ if there are $x_1,\ldots, x_k \in {\cal A}$ such that $f(x_1) = \ldots = f(x_k)=1$. 
\item $\tilde{f}(x)=0$ otherwise. 
\end{enumerate}
We now make two claims about our construction $\tilde{f}$. 
\begin{claim}~\label{clm:tildef-1}
For any point $z \in {\cal A}$, $f(z) = \tilde{f}(z)$. 
\end{claim} 
\begin{proof}
Note that for points $z \in {\cal A}$ where $f(z)=1$, $\tilde{f}(z)=1$ by construction. Further, $\tilde{f}(z)=1$ iff there are points $x_1, \ldots, x_k \in {\cal A}$ such that $f(x_1) = \ldots = f(x_k)=1$. Since ${\cal A}$ does not contain any \textsf{UC}-violating tuple, it follows that if $f(z) =0$, then $\tilde{f}(z) =0$. 
\end{proof}
\begin{claim}~\label{clm:tildef-2}
The function $\tilde{f}$ is union-closed. 
\end{claim}
\begin{proof}
Towards contradiction, let $(y_1, \ldots, y_k, z)$ be a \textsf{UC}-violating tuple. This means that for each $1 \le j \le k$, $\tilde{f}(y_j)=1$. By construction of $\tilde{f}$, this means that for each $j$, there are points $y_{j,1}, \ldots, y_{j, \ell_j}$ such that (i) $f(y_{j_1}) = \ldots = f(y_{j, \ell_j}) =1$;  (ii)  $y_j = \cup_{1 \le i \leq \ell_j} y_{j,i}$. 

This means that $z = \cup_{j=1}^k y_j =  \cup_{j=1}^{k} \cup_{i=1}^{\ell_j} y_{j,i}$ 
and for all $1 \le j \le k$ and $1 \le i \le \ell_j$, $f(y_{j,i})=1$. By construction, this implies that $\tilde{f}(y)=1$, contradicting the assumption that $(y_1, \ldots, y_k, z)$ is a \textsf{UC}-violating tuple.
%\begin{itemize}
%\item 
%\item $y_j = \cup_{1 \le i \leq \ell_j} y_{j,i}$. 
%\end{itemize}
\end{proof}


%Define a tuple $(x_1, \ldots, x_T)$ to be a \rnote{let's tell the reader what this is an abbreviation for, if we can figure it out} $\mathsf{MI}$-tuple if for every $1 < j \le T$, 
%$
%\cup_{1 \le \ell \le j-1} x_i \subsetneq \cup_{1 \le \ell \le j} x_i. 
%$ Note that for any $\mathsf{MI}$-tuple, $T \le n$. 

%Consider a directed hypergraph $G = (V,E)$ where the vertex set $V = \{0,1\}^n$. Given the function $f$ on the hypercube, for  \textsf{UC}-violating minimal tuple $(x_1, \ldots, x_k, x_1\cup \ldots \cup x_k)$, put an edge $e$. 
%Further, for every $\mathsf{MI}$-tuple $(x_1, \ldots, x_T)$, we put a hyperedge $e$ defined as \rnote{nitpick - this is a set and not a sequence, right?}
%\[
%e:= (x_1,\ldots,x_T, \ x_1 \cup x_2, \  x_1 \cup x_2 \cup x_3, \  \ldots, \ x_1 \cup x_2 \cup x_3 \ldots \cup x_T)
%\]
%in the set $E$. Color a hyperedge $e$ as ``red" if the following holds: For some $j>1$, $f(x_1 \cup \ldots \cup x_j) =0$, $f(x_1 \cup \ldots \cup x_{j-1}) =1$ and $f(x_j)=1$.  Otherwise, color the hyperedge $e$ ``blue". Note that a red hyperedge exhibits a \textsf{UC}-violating triple. 
%For any $f: \{0,1\}^n \rightarrow \{0,1\}$ and subset ${\cal A} \subseteq \{0,1\}^n$, let $f_{\cal A}: {\cal A} \rightarrow \{0,1\}$ denote the restriction of $f$ to the set ${\cal A}$.  The next claim states that if the 
%subgraph of $G$ induced by the vertex set ${\cal A}$ does not have any hyperedges, then the function $f_{\cal A}$ can be extended to a union-closed function. 
%\begin{claim}~\label{clm:extension}
%Suppose for  $f: \{0,1\}^n \rightarrow \{0,1\}$ and subset ${\cal A} \subseteq \{0,1\}^n$, the following holds: for every hyperdge in the graph $G$, it contains at least one vertex in $\overline{A}$. 
 %Then, there is a function $\tilde{f}: \{0,1\}^n \rightarrow \{0,1\}$ such that 
%(i) $\tilde{f}(x) = f(x)$ for all $x \in {\cal A}$ and (ii) the function $\tilde{f}$ is union-closed. 
%\end{claim} 
%\begin{proof}
%Note that since the graph $G$ does not have a hyperedge contained entirely in the vertices of ${\cal A}$, it means that there is no $\mathsf{UC}$-violating tuple all of whose coordinates are contained in ${\cal A}$. 



%We show how starting with the set ${\cal A}$, we can add an element to ${\cal A}$ to get a new set ${\cal B}$ and can define a function $\tilde{f}:{\cal B} \to \zo$ such that $f(x) = \tilde{f}(x)$ for all $x \in {\cal A}$ in such a way that the function $\tilde{f}$ has no $\mathsf{UC}$-violating tuple. By iterating this construction, we get the claim. 
%~\\ 
%For a point $z \in \{0,1\}^n \setminus {\cal A}$, define $\mathsf{Con}_{z,{\cal A}}$ as 
%$$ 
%\mathsf{Con}_{z,{\cal A}}= \{(x_1, \ldots, x_T,z): (x_1, \ldots, x_T, z) \textrm{ is a minimal UC-violating tuple} \}
%$$
%Define a point $z \in \{0,1\}^n \setminus {\cal A}$ as {\em conflict-free} if $\mathsf{Con}_{z,{\cal A}} = \emptyset$.  
%\begin{enumerate}
%\item Suppose there exists  $z \in \{0,1\}^n \setminus {\cal A}$
%such that $z$ is conflict-free. 
%Then, we set ${\cal B} = {\cal A} \cup z$ and set $\tilde{f}(z) =0$. Note that by construction, this cannot create a ${\mathsf{UC}}$-violation. 
 %such that there are no $x_1, \ldots, x_T \in {\cal A}$ which satisfy $z = x_1 \cup x_2 \ldots \cup x_T$. In that case, we set  Note that this cannot create a new  because there are no $x_1, \ldots, x_T \in {\cal A}$ such that $z= x_1 \cup x_2 \ldots \cup x_T$. 
%\item Otherwise, choose a $z$ which is not conflict-free. In that case, set ${\cal B} = {\cal A} \cup z$ and set $\tilde{f}(z) =1$. The only way this can create a $\mathsf{UC}$-violation is if there are points $x_1, \ldots, x_{L} \in {\cal A}$ which meet the following conditions: 
%\begin{itemize}
%\item $x_1 \cup x_2 \ldots \cup x_{L-1} \cup z = x_L$; 
%\item $f(x_1) = \ldots =f(x_{L-1}) =1$ and $f(x_L)=0$. 
%\end{itemize}
%However, note that $z$ is not  conflict-free. This means that there are points $y_1, \ldots, y_M \in {\cal A}$ such that $z = y_1 \cup \ldots \cup y_M$ and $f(y_1) = \ldots = f(y_M) =1$. 
%This implies that 
%\[
%\cup_{j=1}^{M} y_j \  \cup_{\ell=1}^{L-1} x_\ell = x_L \  \ \textrm{and} \  \ f(x_L)=0. 
%\]
%Thus, the tuple $(x_1, \ldots, x_{L-1}, y_1, \ldots, y_M)$ is a
%$\mathsf{UC}$-violating tuple. This contradicts the assumption the ${\cal A}$ does not have $\mathsf{UC}$-violating tuples. 
%\end{enumerate} 
%Thus, in either case, we can get a new set ${\cal B}$ such that $|{\cal B} | =|{\cal A}|+1$ and the extension ${\tilde{f}}$ is union-closed.  
%This concludes the proof of \Cref{clm:extension}.
 %Now, suppose $z$ is a point in $\{0,1\}^n \setminus {\cal A}$ such that $z = x_1 \cup \ldots \cup x_T$ where each $x_i \in {\cal A}$. In this case, we define 
%\end{proof} 
 Consequently, there is a union-closed function $\tilde{f}$ which disagrees with $f$ only on the coordinates in ${\cal B}$. Since 
$\duc(f) > \epsilon$, it implies that $|{\cal B}| > \epsilon \cdot 2^n$. This proves  \Cref{lem:distance-uc}. \rnote{This is the end of the proof of \Cref{lem:distance-uc}, right?}
\end{proof}

We next record the following simple claim, the proof of which is left to the reader. 
\begin{claim}~\label{claim:zeroing}
Let $f: \zo^n \rightarrow \zo$. For $0<\epsilon<1$, define $T:=\sqrt{n \cdot 2 \ln (4/\epsilon)}$ and define $f_{\mathsf{trunc}}: \zo^n \rightarrow \zo$ as 
\[
f_{\mathsf{trunc}}(x) = \begin{cases} 0  \ \ &\textrm{if} \  \Vert x \Vert_1 \le n/2 - T; \\
1 \ \ &\textrm{if} \  \Vert x \Vert_1 \ge n/2 + T; \\
f(x) \ \ &\textrm{otherwise}
\end{cases}
\]
Then, the following hold: (i) If $f$ is union-closed, then so is $f_{\mathsf{trunc}}$. (ii)  If $\duc(f)\ge\epsilon$, then $\duc(f_{\mathsf{trunc}}) \ge\epsilon/2$. Finally, (iii) If $(y_1, \ldots, y_T,y_{T+1})$ is a $\mathsf{UC}$-violating tuple for $f_{\mathsf{trunc}}$, then for each $i \in [T+1]$, the point $y_i$ lies in ${[n]\choose j}$
for some $j \in [n/2-T, n/2+T]$. 
\end{claim}

\begin{algorithm}[t]
\caption{Algorithm to test union-closedness}
\label{alg:union-closed}
\vspace{0.5em}
\textbf{Input:} Oracle access to $f: \{0,1\}^n \rightarrow \{0,1\}$, parameter $0 < \eps < 1$\\[0.5em]
\textbf{Output:} ``Union-closed'' or  ``$\eps$-far from Union-closed''

\ 

\textsf{Union-closed-tester}$(f)$:
\begin{enumerate}
\item Repeat the following $M:= 100/\epsilon$ times $\{$
    \item \hspace*{7pt} Set $I:= [n/2 - \sqrt{n \cdot 2 \ln (4/\epsilon)}, n/2 + \sqrt{n  \cdot 2 \ln (4/\epsilon)}].$ 
    \item \hspace*{7pt} Sample $\bx$ uniformly from the set ${[n]\choose I}$. 
    \item \hspace*{7pt} Let $\bx_{\downarrow}:= \{y \le \bx: y \in {[n]\choose I}\}$. Query $f(y)$ for every $y$ in $\bx_{\downarrow}$. 
    \item \hspace*{7pt} 
    Check if there are $y_1, \ldots, y_T \in \bx_{\downarrow}$ such that $(y_1, \ldots, y_T, \bx)$ is a \textsf{UC}-violating tuple. 
    \item \hspace*{7pt}  If yes, output ``$\eps$-far from Union-closed". $\}$
    \item  Output ``Union-closed". 
\end{enumerate}
\end{algorithm}

\Cref{alg:union-closed} gives our algorithm for testing union-closedness, and the following theorem establishes its performance and correctness:

\begin{theorem}~\label{thm:Union-closed-algorithm}
Given oracle access to $f: \zo^n \rightarrow \zo$ and error parameter $\epsilon>0$, the algorithm \textsf{Union-closed-tester} has the following guarantee: 
\begin{enumerate}
\item The algorithm makes $n^{O(\sqrt{n \log (1/\epsilon)})}/\eps$ queries to $f$. 
\item If the function $f$ is union-closed, then the algorithm returns ``Union-closed" with probability $1$. 
\item If $\duc(f) > \epsilon$, then the algorithm returns ``far-from Union-closed" with probability at least $0.9$. 
\end{enumerate}
\end{theorem}
\begin{proof}
Note that for any $x \in {[n]\choose I}$, $|x_{\downarrow}| = n^{O(\sqrt{n \log (1/\epsilon)})}$. Item~1 now follows immediately. 

Item~2 is also immediate, because if $f$ is union-closed, then in Step~5, the algorithm must fail to find a $\mathsf{UC}$-violating tuple, and hence it will always output ``Union-closed" in Step~7. 

Finally, to prove Item~3, note that if $\duc(f) > \epsilon$,  then by \Cref{claim:zeroing} we have $\duc(f_{\mathsf{trunc}}) > \epsilon/2$. Let us call a point $x \in \zo^n$ a ``witness" if there exists $\{y_i\}_{1 \le i \le T}$ such that $(y_1, \ldots, y_T, x)$ is a $\mathsf{UC}$-violating tuple for $f_{\mathsf{trunc}}$. By Claim~\ref{claim:zeroing}, note that any such $x$ and the corresponding $y_1, \ldots, y_T$ must lie in $ {[n]\choose I}$.

Applying~\Cref{lem:distance-uc}, the probability that $\bx$ sampled in Step~3 is a witness is at least $\epsilon/2$. Further, if $x$ is a witness, then in Step~5, the algorithm will find a $\mathsf{UC}$-violating tuple $(y_1, \ldots, y_T, x)$. Thus each iteration of lines 2-7 in the algorithm will output ``far-from Union-closed" with probability at least $\epsilon/2$. This means that repeating the procedure $M=100/\epsilon$ times, we get the correct answer with probability at least $0.9$. 
\end{proof}


\subsubsection{Extension to a triple tester}

The algorithm in Theorem~\ref{thm:Union-closed-algorithm} 
checks for \textsf{UC}-violating tuples. As stated in the introduction, our algorithm can be modified into a so-called ``triple tester" -- i.e., the algorithm checks for \textsf{UC}-violating triples in $f$. In other words, it looks for triples $(y_1, y_2,x)$ such that $f(x)=0$, $f(y_1) = f(y_2) =1$ and $y_1 \cup y_2 =x$. Here, we sketch how this modification is done. 


Given any function $f: \zo^n \rightarrow \zo$ and a corresponding \textsf{UC}-violating tuple $\tau$ defined as $\tau=(x_1, \ldots, x_k, x_1 \cup \ldots \cup x_k)$, we define its augmentation $\widetilde{\tau}$ as
\[
\widetilde{\tau} = (x_1, \ldots, x_k, x_1 \cup x_2, x_1 \cup x_2 \cup x_3, \ldots, x_1 \cup \ldots  \cup x_k). 
\]
Note that whenever $\tau$ is  \textsf{UC}-violating tuple, there is some choice of $1 \le j <k$, such that $(x_1\cup \ldots \cup x_j, x_{j+1}, x_1\cup \ldots \cup x_{j+1})$ is a \textsf{UC}-violating triple. 
 We now have the following easy but crucial observation. 
\begin{fact}~\label{fact:augmented}
Given  \textsf{UC}-violating tuples $\tau_1, \ldots, \tau_M$ such that the augmentations $\widetilde{\tau_1}, \ldots, \widetilde{\tau_M}$ are pairwise-disjoint, we get $N$ \textsf{UC}-violating triples $\sigma_1, \ldots, \sigma_M$. Further, if all the coordinates of the tuples 
$\tau_1, \ldots, \tau_M$ lie in $\binom{[n]}{I}$ for an interval $I$, then so do the coordinates of $\sigma_1, \ldots, \sigma_M$. 
\end{fact}
We next have the following analogue of Lemma~\ref{lem:distance-uc}. 
\begin{lemma}~\label{lem:distance-uc1}
Suppose $f: \{0,1\}^n \rightarrow \{0,1\}$ is such that $\duc(f) > \epsilon$. Then, $f$ has at least $\epsilon/n \cdot 2^n$ many  disjoint \textsf{UC}-violating
tuples. 
\end{lemma}
\begin{proof}
Let ${\cal C}$ be a maximal collection of disjoint \textsf{UC}-violating
tuples for $f$. Let ${\cal B}$ be the set of all points in $\zo^n$ which appear in any of tuples in ${\cal B}$. Note that any violating tuple for $f$ must have at least one of its coordinates in ${\cal B}$. 

With the definition of ${\cal B}$, if we define ${\cal A}$ and $\tilde{f}$ exactly as in the proof of Lemma~\ref{lem:distance-uc}, then the proofs of Claim~\ref{clm:tildef-1} and Claim~\ref{clm:tildef-2} will go through and we will obtain that $\tilde{f}$ is union-closed. Since $\duc(f) > \epsilon$, it follows that $|{\cal B}| > \epsilon \cdot 2^n$ and thus, $|{\cal C}| > \epsilon/n \cdot 2^n$. This finishes the proof. 
\end{proof}

Using Fact~\ref{fact:augmented} and Lemma~\ref{lem:distance-uc1}, it follows that if $\duc(f) >\epsilon$, then $f$ has at least $\epsilon/ n \cdot 2^n$ disjoint violating triples. 



\rnote{Shall we state and prove a claim giving a ``triple tester'' and arguing that it has the same performance guarantee?  This would require us to argue that there are ``many'' disjoint violating triples.  The current exposition in the introduction says that our tester is (or is equivalent to) a simple ``triple tester'' so it might be nice to include this (someone might also find it interesting that there is a triple tester).}

\subsection{Upper bounds for testing intersectingness}

We start with some useful definitions for intersecting sets, and then give our tester for intersecting functions. 

\begin{definition}\label{def:intersecting-violation}
For a function $f: \zo^n \rightarrow \zo$, a pair $(x,y)$ is said to be an \emph{intersection violation} (which we abbreviate ``$\mathsf{I}$-violation'')  if $f(x) = f(y)=1$ and $x \cap y = \emptyset$. 
\end{definition}

Given $f: \zo^n \to \zo$, we write $\dint(f)$ to denote the distance from $f$ to the property which consists of all intersecting functions, i.e.~
\[
\dint(f) = \min_{g: \zo^n \to \zo \text{~is~intersecting}} \dist(f,g).
\]
Similar in spirit to \Cref{lem:distance-uc}, the following lemma shows that any function which is far from intersecting must have many disjoint violating pairs:


\begin{lemma}~\label{lemma:distance-intersecting}
If $f: \zo^n \rightarrow \zo$ has $\dint(f)>\epsilon$, then $f$ has at least $(\epsilon/2) \cdot 2^n$ disjoint $\mathsf{I}$-violation pairs.\rnote{Should the $1/2$ on the RHS be there or no?}
\rnote{Maybe we can replace this lemma statement and proof with \Cref{lem:dist-to-intersecting} and its proof - I think they are equivalent statements, right (other than that \Cref{lemma:distance-intersecting} leaves out the easy reverse direction)?}
\end{lemma}

\begin{proof}
Consider the graph $G = (V,E)$ where $V =\zo^n$ and for every $\mathsf{I}$-violation $(x,y)$, there is an edge between $x$ and $y$. 
We now make a claim for intersecting functions which is analogous to Claim~\ref{clm:extension}: 

\begin{claim}~\label{claim:intersecting-extension}
Suppose for $f: \zo^n \rightarrow \zo$ and a subset ${\cal A} \subseteq \zo^n$, the following holds: any edge in the graph $G$  contains at least one vertex in ${\overline{\cal A}}$. Then there is a function $\tilde{f}: \zo^n \rightarrow \zo$ such that (i) $\tilde{f}(x) = f(x)$ for all $x \in {\cal A}$ and (ii) the function $\tilde{f}$ is intersecting. 
\end{claim}
\begin{proof}
The proof is simple:  for every point outside of ${\cal A}$, we simply set $\tilde{f}(x) =0$, and we have $\tilde{f}$ agree with $f$ for all points in ${\cal A}$.
Note that any ${\mathsf{I}}$-violation pairs $(x,y)$ for $\tilde{f}$ must be such that $x, y \in {\cal A}$. However, by our assumption on $f$ and construction of $\tilde{f}$, such a pair cannot exist.  
\end{proof}

Now, consider a maximal matching in the graph $G$. If the size of this matching is $t$, then there is a vertex cover in $G$ of size $2t$ in the graph $G$; call this vertex cover ${\cal A}$. \rnote{For consistency with \Cref{claim:intersecting-extension}, should this ``${\cal A}$'' be $\overline{\cal A}$?} By applying Claim~\ref{claim:intersecting-extension}, we get that $\dint(f) \le 2t/2^n$. Thus, $t \ge (\epsilon/2) \cdot 2^n$. This finishes the proof of~\Cref{lemma:distance-intersecting}.
\end{proof}

Similar to \Cref{claim:zeroing}, the following claim says that for any $f$, we can truncate $f$ to its middle layers and distance to intersectingness is essentially preserved. It admits a simple proof which we leave to the reader. 
\begin{claim}~\label{claim:zeroing-inter}
Let $f: \zo^n \rightarrow \zo$. For $0<\epsilon<1$, define $T:=\sqrt{n \cdot 2\ln (4/\epsilon)}$ and define $f_{\mathsf{trunc}}: \zo^n \rightarrow \zo$ as 
\[
f_{\mathsf{trunc}}(x) = \begin{cases} 0  \ \ &\textrm{if} \  \Vert x \Vert_1 \le n/2 - T; \\
0 \ \ &\textrm{if} \  \Vert x \Vert_1 \ge n/2 + T; \\
f(x) \ \ &\textrm{otherwise}
\end{cases}
\]
Then, the following hold: (i) If $f$ is intersecting, then so is $f_{\mathsf{trunc}}$. (ii)  If $\dint(f)\ge\epsilon$, then $\dint(f_{\mathsf{trunc}}) \ge\epsilon/2$. Finally, (iii) If $(x,y)$ is a $\mathsf{I}$-violating pair for $f_{\mathsf{trunc}}$, then each of $x$ and $y$ lies in ${[n]\choose j}$
for some $j \in [n/2-T, n/2+T]$. 
\end{claim}

\begin{algorithm}[t]
\caption{Algorithm to test intersectingness}
\label{alg:intersecting}
\vspace{0.5em}
\textbf{Input:} Oracle access to $f: \{0,1\}^n \rightarrow \{0,1\}$,
parameter $0 < \eps < 1$\\[0.5em]
\textbf{Output:} ``Intersecting'' or  ``far from Intersecting''

\ 

\textsf{Intersecting-tester}$(f)$:
\begin{enumerate}
\item Repeat the following $M:= 100/\epsilon$ times $\{$
    \item \hspace*{7pt} Set $I:= [n/2 - \sqrt{n \cdot 2\ln (4/\epsilon)}, n/2 + \sqrt{n  \cdot 2\ln (4/\epsilon)}].$ 
    \item \hspace*{7pt} Sample $\bx$ uniformly from the set ${[n]\choose I}$. 
    \item \hspace*{7pt} Let $\overline{\bx}$ be obtained by flipping every bit of $\bx$. 
    \item \hspace*{7pt} Let $\overline{\bx_{\downarrow}}:= \{y \le \overline{\bx}: y \in {[n]\choose I}\}$. Query $f(y)$ for every $y$ in $\overline{\bx_{\downarrow}}$. 
    \item \hspace*{7pt} 
    Check if there is a $y \in \overline{\bx_{\downarrow}}$ such that $f(y) = f(\bx)=1$.  
    \item \hspace*{7pt}  If yes, output ``far from Intersecting". $\}$
    \item  Output ``Intersecting". 
\end{enumerate}
\end{algorithm}



\begin{theorem}~\label{thm:Intersecting-algorithm}
Given oracle access to $f: \zo^n \rightarrow \zo$ and error parameter $0<\eps<1$, the algorithm \textsf{Intersecting-tester} has the following guarantee: 
\begin{enumerate}
\item The algorithm makes $n^{O(\sqrt{n \log (1/\epsilon)})}/\eps$ queries to $f$. 
\item If the function $f$ is intersecting, then the algorithm returns ``Intersecting" with probability $1$. 
\item If $\dint(f) > \epsilon$, then the algorithm returns ``far from Intersecting" with probability at least $0.9$. 
\end{enumerate}
\end{theorem}
\begin{proof}
Note that for any $x \in {[n]\choose I}$, $|\overline{x_{\downarrow}}| = n^{O(\sqrt{n \log (1/\epsilon)})}$. Item~1 now follows immediately. 

Item~2 is also immediate, because if $f$ is intersecting, then in Step~5, the algorithm will fail to find an $\mathsf{I}$-violating pair. Thus, it will always output ``Intersecting" in Step~8. 

Finally, to prove Item~3, note that if $\dint(f) > \epsilon$,  then $\dint(f_{\mathsf{trunc}}) > \epsilon/2$ (where $f_{\mathsf{trunc}}$ is defined in  Claim~\ref{claim:zeroing-inter}). Now, call a point $x \in \zo^n$ a ``witness" if there exists $y \in \zo^n$ such that $(y, x)$ is an $\mathsf{I}$-violating pair for $f_{\mathsf{trunc}}$. By Claim~\ref{claim:zeroing}, note that any such $x$ and the corresponding $y$ must lie in $ {[n]\choose I}$.

Applying~\Cref{lemma:distance-intersecting}, the probability that $\bx$ sampled in Step~3 is a witness is at least $\epsilon/2$. Further, if $x$ is a witness, then in Step~5, the algorithm will find a $\mathsf{I}$-violating pair $(y, x)$. Thus each iteration of lines 2-7 in the algorithm will output ``far from Intersecting" with probability at least $\epsilon/2$. This means that repeating the procedure $M=100/\epsilon$ times, we get the correct answer with probability at least $0.9$. 
\end{proof}

\rnote{Same question/comment as the earlier rnote: shall we state and prove a claim giving a ``pair tester'' and arguing that it has the same performance guarantee?}


==> sections/uc-fig.tex <==
%!TEX root = ../int-uc-tolerant.tex


\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{patterns}

\begin{figure}
\centering

\begin{tikzpicture}[scale=0.9]

	%%%%%%%%%%%%%%% CONTROL SUBCUBE %%%%%%%%%%%%%%%%% 
	
	% colors
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25) -- (0, 3);
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75) -- (0, 3);
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
	
	\fill[color=purple!20!blue!40!white!70] (-2.25, 0.75) -- (-0.5, -1) -- (0, -0.5) -- (0.5, -1) -- (2.25, 0.75) -- (0, 3);
	
	% control cube
	\draw[-] (0, -3) -- (-3, 0) -- (0, 3) -- (3, 0) -- (0, -3);

	
	% talagrand subcubes
	\draw[-] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25);
	\draw[-] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75);
	\draw[-,line width=0.3mm] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
		
	% nodes
	\node (0) at (0, -2){$0$};
	\node (1) at (0, 1){$1$};
	\node (talagrand-cube) at (1.15, -0.85){$\bT_{\ell}$};
	
	
	
	%%%%%%%%%%%%%%%% ACTION SUBCUBE %%%%%%%%%%%%%%%%%
	
	\draw[-] (9, -1.5) -- (7.5, 0) -- (9, 1.5) -- (10.5, 0) -- (9, -1.5);
	
	\node[circle,fill=black,inner sep=0pt,minimum size=1pt,scale=0.35,label=below:{\small$\bs_{\ell}$}] (arr) at (9.25, .15){\small$\bs_{\ell}$};

	
	%%%%%%%%%%%%%%%%%%%% EXTRA GOODIES %%%%%%%%%%%%%%%%
	
	\draw[-latex] (2.34, 0) -- (7, 0);
	\node () at (2.34, 0) [circle,fill,inner sep=1pt]{};
	
	\node (control) at (0, -4.75){$\zo^{\bC} \equiv \zo^m$};
	\node (action) at (9, -4.75){$\zo^{\bA} \equiv \zo^{a}$};
	
	
	
\end{tikzpicture}


\caption*{(a) A draw of $\fyes\sim\Dyes$}

\

\
	
\begin{tikzpicture}[scale=0.9]

	%%%%%%%%%%%%%%% CONTROL SUBCUBE %%%%%%%%%%%%%%%%% 
	
	% colors
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25) -- (0, 3);
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75) -- (0, 3);
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
	
	\fill[color=purple!20!blue!40!white!70] (-2.25, 0.75) -- (-0.5, -1) -- (0, -0.5) -- (0.5, -1) -- (2.25, 0.75) -- (0, 3);
	
	% control cube
	\draw[-] (0, -3) -- (-3, 0) -- (0, 3) -- (3, 0) -- (0, -3);

	
	% talagrand subcubes
	\draw[-] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25);
	\draw[-] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75);
	\draw[-,line width=0.3mm] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
		
	% nodes
	\node (0) at (0, -2){$0$};
	\node (1) at (0, 1){$1$};
	\node (talagrand-cube) at (1.15, -0.85){$\bT_{\ell}$};
	
	
	
	%%%%%%%%%%%%%%%% ACTION SUBCUBES %%%%%%%%%%%%%%%%%
	
	% top
	
	\node (heads) at (5.5, 2.5){\includegraphics[width=1.1cm]{images/quarter-front}};
	\node (bh) at (5.5, 1.5){If $\bb_{\ell} = 1$:};
	
	
	\draw[-] (9, 1) -- (7.5, 2.5) -- (9, 4) -- (10.5, 2.5) -- (9, 1);
	
	\node[circle,fill=black,inner sep=0pt,minimum size=1pt,scale=0.35,label=below:{\small$\br_{\ell}$}] (arr) at (8.5, 2.75){\small$\br_{\ell}$};
	\node (ol-arr)[circle,fill=black,inner sep=0pt,minimum size=1pt,scale=0.35,label=below:{\small$\overline{\br}_{\ell}$}] at (9.5, 2.25){\small $\overline{\br}_{\ell}$};
	
	\draw[dashed] (arr) -- (9, 4) -- (ol-arr);

	
	% bottom
	
	\node (tails) at (5.5, -2){\includegraphics[width=1.1cm]{images/jersey-quarter-back}};
	\node (bt) at (5.5, -3){If $\bb_{\ell} = 0$:};
	
	\draw[-] (9, -3.5) -- (7.5, -2) -- (9, -0.5) -- (10.5, -2) -- (9, -3.5);	
	

	
	%%%%%%%%%%%%%%%%%%%% EXTRA GOODIES %%%%%%%%%%%%%%%%
	
	\draw[-latex] (2.35, 0.1) -- (4.5, 2.25);
	\draw[-latex] (2.35, 0.1) -- (4.5, -2.25);
	\node () at (2.35, 0.1) [circle,fill,inner sep=1pt]{};
	
	\node (control) at (0, -4.75){$\zo^{\bC} \equiv \zo^m$};
	\node (action) at (9, -4.75){$\zo^{\bA} \equiv \zo^{a}$};
	
	
	
\end{tikzpicture}

\caption*{(b) A draw of $\fno\sim\Dno$}
	
	\caption{The left hand side depicts the control subcube $\zo^{\bC}$ with the terms of the Talagrand DNF, and the right hand side depicts an action subcube $\zo^{\bA}$. The cross-hatched region in the control subcube corresponds to assignments that are satisfied by a unique Talagrand term $\bT_\ell$.}
	\label{fig:uc-no-dist}
\end{figure}

==> sections/uc-old.tex <==
%!TEX root = ../int-uc-tolerant.tex

\section{Testing Union-Closed Families}
\label{sec:union}

In this section, we prove a $n^{\Omega(\log(1/\epsilon))}$-query lower bound against non-adaptive algorithms for testing union-closedness (with either one-sided or two-sided error). More formally, we establish the following:

\begin{theorem} \label{thm:uc-lb}
	Let $\eps \in [2^{-\sqrt{n}}, c]$ for some absolute constant $c > 0$. Then any non-adaptive algorithm that tests whether a function $f\isazofunc$ is union-closed or is $\epsilon$-far from union-closed must make $n^{\Omega\pbra{\log(1/\eps)}}$ many queries to $f$.
\end{theorem}

We describe the hard distributions in \Cref{subsec:uc-yes-no-dists} and then prove \Cref{thm:uc-lb} in \Cref{subsec:uc-indistinguish}

\subsection{The $\Dyes$ and $\Dno$ Distributions}
\label{subsec:uc-yes-no-dists}


Our construction of the hard distributions $\Dyes$ and $\Dno$ are inspired by the constructions for the lower bound against intersectingness testing in \Cref{sec:intersecting}; in particular, our hard functions will also comprise of a truncated Talagrand random DNF on a set of ``control bits'' $\bC$, and then a function tailored to the union-closedness property on a set of ``action bits'' $\bA$. We start by describing the $\Dyes$ distribution:


\begin{definition} \label{def:uc-yes}
	Given $\eps > 0$, a draw of a Boolean function $\fyes \isazofunc$ from the distribution $\Dyes := \Dyes(n,\eps)$ is obtained as follows:
	\begin{enumerate}
		\item Draw a random set of $a := \log(1/\eps)$ coordinates $\bA \sse[n]$, i.e. 
		\[\bA \sim {[n]\choose a}, \qquad\text{and set}\qquad \bC := [n]\setminus \bA.\]
		Let $c := |\bC| = n-a$.
		\item Let $L :=0.1\cdot2^{2\sqrt{c}}$ and draw an $L$-term monotone Talagrand DNF $\bT\sim \Tal(c, 0.5)$ as defined in \Cref{def:talagrand} on $\zo^{\bC}$. 
		\item For each $\ell\in[L]$, independently draw a uniformly random $a$-bit string $\bs(\ell) \in \zo^{\bA}$. 
		\item Output the function 
		\begin{equation*} \label{eq:uc-yes}
			\fyes(x_{\bC}, x_{\bA}) := 
			\begin{cases}
				1 & |S_{\bT}(x_{\bC})| \geq 2 \\
				\Indicator\cbra{x_{\bA} = \bs(\ell)} & S_{\bT}(x_{\bC}) = \{\ell\}\\
				0 & |S_{\bT}(x_{\bC})| = 0
			\end{cases}
		\end{equation*}
		where $S_{\bT}$ is as defined in \Cref{notation:term-count}.
	\end{enumerate}
\end{definition}



We verify that functions drawn from $\Dyes$ are indeed union-closed:

\begin{claim} \label{claim:uc-yes-indeed-yes}
	Every function $\fyes \sim \supp(\Dyes)$ is union-closed.
\end{claim}

\begin{proof}
	Let $\fyes$ be as in \Cref{def:uc-yes}. We will show the following:
	\[\text{If}~ \fyes(x) = \fyes(y) = 1,~\text{then}~\fyes(x\cup y) = 1.\]
	For brevity we denote $z:= x \cup y$. Now, note that if $\fyes(x) = 1$, then either 
	\begin{enumerate}
		\item[(a)] $|S_{\bT}(x_{\bC})| \geq 2$; or 
		\item[(b)] $S_{\bT}(x_{\bC}) = \{\ell\}$ for some $\ell\in[L]$ and $x_{\bA} = \bs(\ell)$,
	\end{enumerate}
	with analogous statements holding for $y$. Note that if (a) holds for either $x$ or $y$, then $|S_{\bT}(z_{\bC})| \geq 2$ and so $\fyes(z) = 1$. We therefore only have to consider the case when (b) holds for both $x$ and $y$. Indeed, suppose that 
	\[S_{\bT}(x_{\bC}) = \{\ell_1\} \qquad\text{and}\qquad S_{\bT}(y_{\bC}) = \{\ell_2\}.\]
	If $\ell_1\neq\ell_2$, then $\{\ell_1, \ell_2\} \sse S_{\bT}(z_{\bC})$ and so $\fyes(z) = 1$. On the other hand, if $\ell_1 = \ell_2$ then either (i) $S_{\bT}(z_{\bC}) = \{\ell_1\}$, in which case as $\bs(\ell_1) = x_{\bA} = y_{\bA} = z_{\bA}$ we will have $\fyes(z) = 1$; or (ii) $|S_{\bT}(z_{\bC})|\geq 2$and so $\fyes(z) = 1$. It follows that $\fyes$ is union closed.
\end{proof}

We now turn to a description of the $\Dno$ distribution; see \Cref{fig:uc-no-dist} for an illustration of the construction. 

\begin{definition} \label{def:uc-no}
\rnote{Some range on allowable $\eps$-values --- maybe at least $1/2^{\sqrt{n}}$, check this}
	Given $\eps > 0$, a draw of a Boolean function $\fno \isazofunc$ from the distribution $\Dno := \Dno(n,\eps)$ is obtained as follows:
	\begin{enumerate}
		\item Draw a random set of $a := \log(1/\eps)$ coordinates $\bA \sse[n]$, i.e. 
		\[\bA \sim {[n]\choose a}, \qquad\text{and set}\qquad \bC := [n]\setminus \bA.\]
		Let $c := |\bC| = n-a$.
		\item Let $L :=0.1\cdot2^{2\sqrt{c}}$ and draw an $L$-term monotone Talagrand DNF $\bT\sim \Tal(c, 0.5)$ as defined in \Cref{def:talagrand} on $\zo^{\bC}$. 
		\item For each $\ell\in[L]$, independently draw a uniformly random $a$-bit string $\br(i) \in \zo^{\bA}$ as well as a uniformly random bit $\bb(i) \in \zo$. 
		\item Output the function 
		\begin{equation*} \label{eq:uc-yes}
			\fyes(x_{\bC}, x_{\bA}) := 
			\begin{cases}
				1 & |S_{\bT}(x_{\bC})| \geq 2 \\
				\bb(\ell)\cdot\Indicator\cbra{x_{\bA} \in \{\br(i), \overline{\br}(i)\}} & S_{\bT}(x_{\bC}) = \{\ell\}\\
				0 & |S_{\bT}(x_{\bC})| = 0
			\end{cases}
		\end{equation*}
		where $\overline{\br}(i) := 1^a - \br(i)$ is the antipode of $\br(i)$. 
	\end{enumerate}
\end{definition}

\begin{figure}
	\centering
	
	{\large \red{TODO: Update picture to show that the DNF is monotone.}}
	
%	\begin{tikzpicture}
%		\node[inner sep=0pt] (uc-no-dist) at (0,0) {\includegraphics[width=0.9\textwidth]{images/uc-no.png}};
%		
%		\node (control-cube) at (-4.45, -4.25) {$\zo^{\bC}$};
%		\node (term) at (-5.05, 1.35) {$\bT_i$};
%		\node (action-cube) at (5.85, -4.25) {$\zo^{\bA}$};
%		\node (new-jersey) at (2.05, -4.25) {$\bb(i)$};
%		
%		\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=4pt, label=below:{$\br(i)$}] (tails-0) at (5, 2.25) {};
%		\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=4pt, label=below:{$\overline{\br}(i)$}] (tails-1) at (6.4, 1.85) {};
%		\node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] (tails-2) at (5.5, 2.75) {};
%		\draw[dashed] (tails-0) -- (tails-2) -- (tails-1);
%		
%%		\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=4pt, label=below:{$\br(i)$}] (tails-0) at (4.25, -2.75) {};
%	\end{tikzpicture}
	
	\caption{The $\Dno$ distribution for the union-closedness testing lower bound. The blue regions in the control cube $\zo^{\bC}$ correspond to inputs which satisfy a unique term in the Talagrand random DNF $\bT$.}
	\label{fig:uc-no-dist}
\end{figure}

As illustrated by \Cref{fig:uc-no-dist}, we associated each Talagrand term $\bT_i$ with a uniformly random bit $\bb(i)$. If $\bb(i) = 1$ then the action cube comprises of a single union-closedness violation,\footnote{This is with the exception of $\br(i) = 0^a$ or $1^a$; in this case $\br(i) \cup \overline{\br}(i) = 1^a$ and so the function on the action bits will indeed by union-closed. Note, however, that this only happens with probability $1/2^a$.} and if $\bb(i) = 0$ then the action cube has zero satisfying assignments. This ensures that in expectation, the measure of a function drawn from $\Dno$ is indistinguishable from that of a function drawn from $\Dyes.$ 

\begin{claim} \label{claim:uc-no-far-from-uc}
	Let $\eps > \red{TODO}$. With probability \red{$1-o_n(1)$}, a function $\fno\sim\Dno = \Dno(n,\eps)$ satisfies $\dist(\fno, g) \geq \Omega(\eps)$ for every union-closed function $g\isazofunc$.
\end{claim}

\begin{proof}
	\red{TODO: Say that a function is ``nice'' if the number of random coin tosses $\bb(i)$ is roughly what you would expect according to the Chernoff bound.}
\end{proof}







\subsection{Indistinguishability of the Hard Distributions}
\label{subsec:uc-indistinguish}

==> sections/uc.tex <==
%!TEX root = ../int-uc-tolerant.tex

\section{Lower bounds for Testing Union-Closed Families}
\label{sec:union}

In this section, we prove a $n^{\Omega(\log(1/\epsilon))}$-query lower bound against non-adaptive algorithms for testing union-closedness (with either one-sided or two-sided error). More formally, we establish the following:

\begin{theorem} \label{thm:uc-lb}
	Let $\eps \in [2^{-\sqrt{n}}, c]$ for some absolute constant $c > 0$. Then any non-adaptive algorithm that tests whether a function $f\isazofunc$ is union-closed or is $\epsilon$-far from union-closed must make $n^{\Omega\pbra{\log(1/\eps)}}$ many queries to $f$.
\end{theorem}

We describe the hard distributions in \Cref{subsec:uc-yes-no-dists} and then prove \Cref{thm:uc-lb} in \Cref{subsec:uc-indistinguish}.

\subsection{The $\Dyes$ and $\Dno$ Distributions}
\label{subsec:uc-yes-no-dists}


Our construction of the hard distributions $\Dyes$ and $\Dno$ are inspired by the constructions for the lower bound against intersectingness testing in \Cref{sec:intersecting}; in particular, our hard functions will also comprise of a truncated Talagrand random DNF on a set of ``control bits'' $\bC$, and then a function tailored to the union-closedness property on a set of ``action bits'' $\bA$. We start by describing the $\Dyes$ distribution:


\begin{definition} \label{def:uc-yes}
	Given $\eps > 0$, a draw of a Boolean function $\fyes \isazofunc$ from the distribution $\Dyes := \Dyes(n,\eps)$ is obtained as follows:
	\begin{enumerate}
		\item Draw a random set of $a := \log(1/\eps)$ coordinates $\bA \sse[n]$, i.e. 
		\[\bA \sim {[n]\choose a}, \qquad\text{and set}\qquad \bC := [n]\setminus \bA.\]
		Let $c := |\bC| = n-a$.
		\item Let $L :=0.1\cdot2^{2\sqrt{c}}$ and draw an $L$-term monotone Talagrand DNF $\bT\sim \Tal(c, 0.5)$ as defined in \Cref{def:talagrand} on $\zo^{\bC}$. 
		\item For each $\ell\in[L]$, independently draw a uniformly random $a$-bit string $\bs_\ell \in \zo^{\bA}$. 
		\item Output the function 
		\begin{equation*} \label{eq:uc-yes}
			\fyes(x_{\bC}, x_{\bA}) := 
			\begin{cases}
				1 & |S_{\bT}(x_{\bC})| \geq 2 \\
				\Indicator\cbra{x_{\bA} = \bs_\ell} & S_{\bT}(x_{\bC}) = \{\ell\}\\
				0 & |S_{\bT}(x_{\bC})| = 0
			\end{cases}
		\end{equation*}
		where $S_{\bT}$ is as defined in \Cref{notation:term-count}.
	\end{enumerate}
\end{definition}



We verify that functions drawn from $\Dyes$ are indeed union-closed:

\begin{claim} \label{claim:uc-yes-indeed-yes}
	Every function $\fyes \sim \supp(\Dyes)$ is union-closed.
\end{claim}

\begin{proof}
	Let $\fyes$ be as in \Cref{def:uc-yes}. We will show the following:
	\[\text{If}~ \fyes(x) = \fyes(y) = 1,~\text{then}~\fyes(x\cup y) = 1.\]
	For brevity we denote $z:= x \cup y$. Now, note that if $\fyes(x) = 1$, then either 
	\begin{enumerate}
		\item[(a)] $|S_{\bT}(x_{\bC})| \geq 2$; or 
		\item[(b)] $S_{\bT}(x_{\bC}) = \{\ell\}$ for some $\ell\in[L]$ and $x_{\bA} = \bs_\ell$,
	\end{enumerate}
	with analogous statements holding for $y$. Note that if (a) holds for either $x$ or $y$, then $|S_{\bT}(z_{\bC})| \geq 2$ and so $\fyes(z) = 1$. We therefore only have to consider the case when (b) holds for both $x$ and $y$. Indeed, suppose that 
	\[S_{\bT}(x_{\bC}) = \{\ell_1\} \qquad\text{and}\qquad S_{\bT}(y_{\bC}) = \{\ell_2\}.\]
	If $\ell_1\neq\ell_2$, then $\{\ell_1, \ell_2\} \sse S_{\bT}(z_{\bC})$ and so $\fyes(z) = 1$. On the other hand, if $\ell_1 = \ell_2$ then either (i) $S_{\bT}(z_{\bC}) = \{\ell_1\}$, in which case as $\bs_{\ell_1} = x_{\bA} = y_{\bA} = z_{\bA}$ we will have $\fyes(z) = 1$; or (ii) $|S_{\bT}(z_{\bC})|\geq 2$ and so $\fyes(z) = 1$. It follows that $\fyes$ is union closed.
\end{proof}

We now turn to a description of the $\Dno$ distribution; see \Cref{fig:uc-no-dist} for an illustration of the construction. 

\begin{definition} \label{def:uc-no}
\rnote{Some range on allowable $\eps$-values --- maybe at least $1/2^{\sqrt{n}}$, check this}
	Given $\eps > 0$, a draw of a Boolean function $\fno \isazofunc$ from the distribution $\Dno := \Dno(n,\eps)$ is obtained as follows:
	\begin{enumerate}
		\item Draw a random set of $a := \log(1/\eps)$ coordinates $\bA \sse[n]$, i.e. 
		\[\bA \sim {[n]\choose a}, \qquad\text{and set}\qquad \bC := [n]\setminus \bA.\]
		Let $c := |\bC| = n-a$.
		\item Let $L :=0.1\cdot2^{2\sqrt{c}}$ and draw an $L$-term monotone Talagrand DNF $\bT\sim \Tal(c, 0.5)$ as defined in \Cref{def:talagrand} on $\zo^{\bC}$. 
		\item For each $\ell\in[L]$, independently draw a uniformly random $a$-bit string $\br_\ell \in \zo^{\bA}$ as well as a uniformly random bit $\bb_\ell \in \zo$. 
		\item Output the function 
		\begin{equation*} \label{eq:uc-yes}
			\fyes(x_{\bC}, x_{\bA}) := 
			\begin{cases}
				1 & |S_{\bT}(x_{\bC})| \geq 2 \\
				\bb_\ell \cdot\Indicator\cbra{x_{\bA} \in \{\br_\ell, \overline{\br}_\ell\}} & S_{\bT}(x_{\bC}) = \{\ell\}\\
				0 & |S_{\bT}(x_{\bC})| = 0
			\end{cases}
		\end{equation*}
		where $\overline{\br}_\ell := 1^a - \br_\ell$ is the antipode of $\br_\ell$. 
	\end{enumerate}
\end{definition}

%%% FIGURE %%%
\input{sections/uc-fig}

As illustrated by \Cref{fig:uc-no-dist}, we associated each Talagrand term $\bT_i$ with a uniformly random bit $\bb_\ell$. If $\bb_\ell = 1$ then the action cube comprises of a single union-closedness violation,\footnote{This is with the exception of $\br_\ell = 0^a$ or $1^a$; in this case $\br_\ell \cup \overline{\br}_\ell = 1^a$ and so the function on the action bits will indeed be union-closed. Note, however, that this only happens with probability $1/2^a$.} and if $\bb_\ell = 0$ then the action cube has zero satisfying assignments. This ensures that in expectation, the measure of a function drawn from $\Dno$ is indistinguishable from that of a function drawn from $\Dyes.$ 

\begin{claim} \label{claim:uc-no-far-from-uc}
	Let $\eps > \red{TODO}$. With probability \red{$1-o_n(1)$}, a function $\fno\sim\Dno = \Dno(n,\eps)$ satisfies $\dist(\fno, g) \geq \Omega(\eps)$ for every union-closed function $g\isazofunc$.
\end{claim}

\begin{proof}
	\red{TODO: Say that a function is ``nice'' if the number of random coin tosses $\bb_\ell$ is roughly what you would expect according to the Chernoff bound.}
\end{proof}



\subsection{Indistinguishability of the Hard Distributions}

\label{subsec:uc-indistinguish}
